The Tempered Finite Element Method

In this paper, we propose a new approach -- the Tempered Finite Element Method (TFEM) -- that extends the Finite Element Method (FEM) to classes of meshes that include zero-measure or nearly degenerate elements for which standard FEM approaches do not allow convergence. First, we review why the maximum angle condition [2] is not necessary for FEM convergence and what are the real limitations in terms of meshes. Next, we propose a simple modification of the classical FEM for elliptic problems that provably allows convergence for a wider class of meshes including bands of caps that cause locking of the solution in standard FEM formulations. The proposed method is trivial to implement in an existing FEM code and can be theoretically analyzed. We prove that in the case of exactly zero-measure elements it corresponds to mortaring. We show numerically and theoretically that what we propose is functional and sound. The remainder of the paper is devoted to extensions of the TFEM method to linear elasticity, mortaring of non-conforming meshes, high-order elements, and advection.

==> data/CG_alone_D100.tex <==
0.000000 1.00000000000
1.000000 0.54790403160
2.000000 0.40500312225
3.000000 0.31941201694
4.000000 0.27169674282
5.000000 0.24056215303
6.000000 0.21590693286
7.000000 0.20013867404
8.000000 0.19280579183
9.000000 0.19438613281
10.000000 0.19189196092
11.000000 0.17107398163
12.000000 0.16557253000
13.000000 0.17590174848
14.000000 0.14988314477
15.000000 0.13362931448
16.000000 0.12634274283
17.000000 0.12410604646
18.000000 0.11804513037
19.000000 0.10721868597
20.000000 0.09728633281
21.000000 0.08780966481
22.000000 0.08235462755
23.000000 0.08074907136
24.000000 0.07179024598
25.000000 0.06380124433
26.000000 0.05855759620
27.000000 0.05343006340
28.000000 0.04920924739
29.000000 0.04570676594
30.000000 0.04165810593
31.000000 0.03755414510
32.000000 0.03416200397
33.000000 0.03130029163
34.000000 0.02885880651
35.000000 0.02679859248
36.000000 0.02500190327
37.000000 0.02323077621
38.000000 0.02143166941
39.000000 0.01989356405
40.000000 0.01864569193
41.000000 0.01761110668
42.000000 0.01674922817
43.000000 0.01615131985
44.000000 0.01572538967
45.000000 0.01536164863
46.000000 0.01509200718
47.000000 0.01524126985
48.000000 0.01662869933
49.000000 0.01642236176
50.000000 0.01479040666
51.000000 0.01437212043
52.000000 0.01454115375
53.000000 0.01545551198
54.000000 0.01846462570
55.000000 0.02404294094
56.000000 0.02054897498
57.000000 0.00827785620
58.000000 0.00343909546
59.000000 0.00178645005
60.000000 0.00159737124
61.000000 0.00110093705
62.000000 0.00085813353
63.000000 0.00070747830
64.000000 0.00056471875
65.000000 0.00054188004
66.000000 0.00043633930
67.000000 0.00041056253
68.000000 0.00035216740
69.000000 0.00032980889
70.000000 0.00030131092
71.000000 0.00027086393
72.000000 0.00026205839
73.000000 0.00023189524
74.000000 0.00022632662
75.000000 0.00019862911
76.000000 0.00018695838
77.000000 0.00017273360
78.000000 0.00015965611
79.000000 0.00015351894
80.000000 0.00014383958
81.000000 0.00014089496
82.000000 0.00012058214
83.000000 0.00011081489
84.000000 0.00010384572
85.000000 0.00009805110
86.000000 0.00010193352
87.000000 0.00009794550
88.000000 0.00009712457
89.000000 0.00010343698
90.000000 0.00009358985
91.000000 0.00008720510
92.000000 0.00008828097
93.000000 0.00008819977
94.000000 0.00008772302
95.000000 0.00008869328
96.000000 0.00008732081
97.000000 0.00008546014
98.000000 0.00008528493
99.000000 0.00008298257
100.000000 0.00008254501
101.000000 0.00008644671
102.000000 0.00007976325
103.000000 0.00007251862
104.000000 0.00006820027
105.000000 0.00006774041
106.000000 0.00006781043
107.000000 0.00006932599
108.000000 0.00006924350
109.000000 0.00006506325
110.000000 0.00005998324
111.000000 0.00005572218
112.000000 0.00005304220
113.000000 0.00005494152
114.000000 0.00005693624
115.000000 0.00005604657
116.000000 0.00005612984
117.000000 0.00005558912
118.000000 0.00005531715
119.000000 0.00005374143
120.000000 0.00005305955
121.000000 0.00004922275
122.000000 0.00004670526
123.000000 0.00004892140
124.000000 0.00005335128
125.000000 0.00004414637
126.000000 0.00004035973
127.000000 0.00003753925
128.000000 0.00003661521
129.000000 0.00003564036
130.000000 0.00003337869
131.000000 0.00003099926
132.000000 0.00002922941
133.000000 0.00002667925
134.000000 0.00002453111
135.000000 0.00002266544
136.000000 0.00002145598
137.000000 0.00002090052
138.000000 0.00001990963
139.000000 0.00001734507
140.000000 0.00001587012
141.000000 0.00001556530
142.000000 0.00001374889
143.000000 0.00001169489
144.000000 0.00001055524
145.000000 0.00000954408
146.000000 0.00000842731
147.000000 0.00000769001
148.000000 0.00000721994
149.000000 0.00000705535
150.000000 0.00000622617
151.000000 0.00000555285
152.000000 0.00000496606
153.000000 0.00000447210
154.000000 0.00000420519
155.000000 0.00000394465
156.000000 0.00000372305
157.000000 0.00000353891
158.000000 0.00000350772
159.000000 0.00000382676
160.000000 0.00000346473
161.000000 0.00000298071
162.000000 0.00000272016
163.000000 0.00000256301
164.000000 0.00000249488
165.000000 0.00000240470
166.000000 0.00000229188
167.000000 0.00000204432
168.000000 0.00000182906
169.000000 0.00000164294
170.000000 0.00000148107
171.000000 0.00000138063
172.000000 0.00000134601
173.000000 0.00000124898
174.000000 0.00000116962
175.000000 0.00000115167
176.000000 0.00000112505
177.000000 0.00000108710
178.000000 0.00000102146
179.000000 0.00000098333
180.000000 0.00000091775
181.000000 0.00000085481
182.000000 0.00000089903
183.000000 0.00000088673
184.000000 0.00000074469
185.000000 0.00000069617
186.000000 0.00000069681
187.000000 0.00000067866
188.000000 0.00000063742
189.000000 0.00000061028
190.000000 0.00000058158
191.000000 0.00000054727
192.000000 0.00000054296
193.000000 0.00000058358
194.000000 0.00000048652
195.000000 0.00000043978
196.000000 0.00000041216
197.000000 0.00000038847
198.000000 0.00000035559
199.000000 0.00000033568
200.000000 0.00000033005
201.000000 0.00000031519
202.000000 0.00000029141
203.000000 0.00000027375
204.000000 0.00000025979
205.000000 0.00000024890
206.000000 0.00000024478
207.000000 0.00000023374
208.000000 0.00000022359
209.000000 0.00000021045
210.000000 0.00000019736
211.000000 0.00000017622
212.000000 0.00000014752
213.000000 0.00000013143
214.000000 0.00000011978
215.000000 0.00000010463
216.000000 0.00000008843
217.000000 0.00000007563
218.000000 0.00000006647
219.000000 0.00000005887
220.000000 0.00000005481
221.000000 0.00000004979
222.000000 0.00000004510
223.000000 0.00000004088
224.000000 0.00000003850
225.000000 0.00000003855
226.000000 0.00000004281
227.000000 0.00000003878
228.000000 0.00000003610
229.000000 0.00000003867
230.000000 0.00000003438
231.000000 0.00000002885
232.000000 0.00000002608
233.000000 0.00000002466
234.000000 0.00000002350
235.000000 0.00000002139
236.000000 0.00000001837
237.000000 0.00000001558
238.000000 0.00000001286
239.000000 0.00000001045
240.000000 0.00000000900
241.000000 0.00000000766
242.000000 0.00000000688
243.000000 0.00000000641
244.000000 0.00000000584
245.000000 0.00000000537
246.000000 0.00000000493
247.000000 0.00000000462
248.000000 0.00000000425
249.000000 0.00000000377
250.000000 0.00000000329
251.000000 0.00000000303
252.000000 0.00000000255
253.000000 0.00000000206
254.000000 0.00000000173
255.000000 0.00000000143
256.000000 0.00000000121
257.000000 0.00000000103
258.000000 0.00000000092
259.000000 0.00000000087
260.000000 0.00000000084
261.000000 0.00000000072
262.000000 0.00000000061
263.000000 0.00000000054
264.000000 0.00000000048
265.000000 0.00000000044
266.000000 0.00000000041
267.000000 0.00000000037
268.000000 0.00000000034
269.000000 0.00000000030
270.000000 0.00000000025
271.000000 0.00000000021
272.000000 0.00000000020
273.000000 0.00000000018
274.000000 0.00000000015
275.000000 0.00000000012
276.000000 0.00000000011
277.000000 0.00000000009


==> data/CG_alone_D1000.tex <==
0.000000 1.00000000000
1.000000 0.51435782419
2.000000 0.37327581978
3.000000 0.48951813258
4.000000 0.35280713692
5.000000 0.37625495898
6.000000 0.30970019136
7.000000 0.39537365746
8.000000 0.25315770159
9.000000 0.37137034322
10.000000 0.26051554100
11.000000 0.26798224126
12.000000 0.33444340198
13.000000 0.22401435711
14.000000 0.28299312212
15.000000 0.26952094960
16.000000 0.21910508920
17.000000 0.26028761291
18.000000 0.24231997969
19.000000 0.21324380789
20.000000 0.23106610783
21.000000 0.23276633533
22.000000 0.18787498484
23.000000 0.23404045690
24.000000 0.19899382213
25.000000 0.17721781166
26.000000 0.20963951891
27.000000 0.17433112183
28.000000 0.17621828470
29.000000 0.17935526752
30.000000 0.16084113485
31.000000 0.15535973710
32.000000 0.16162334433
33.000000 0.14356606678
34.000000 0.14193117658
35.000000 0.13972124239
36.000000 0.13027681513
37.000000 0.12711459517
38.000000 0.12211691821
39.000000 0.11581170077
40.000000 0.11198078417
41.000000 0.10687343102
42.000000 0.10600903076
43.000000 0.09606486073
44.000000 0.09841753831
45.000000 0.08955482716
46.000000 0.08458330300
47.000000 0.08449475915
48.000000 0.08176251817
49.000000 0.07326119198
50.000000 0.07478096539
51.000000 0.07253948903
52.000000 0.06561961805
53.000000 0.06800421538
54.000000 0.06443405404
55.000000 0.05765903368
56.000000 0.06119560344
57.000000 0.05277540250
58.000000 0.05599697770
59.000000 0.04975158070
60.000000 0.04874748283
61.000000 0.04876135830
62.000000 0.04484659108
63.000000 0.04299227001
64.000000 0.04400959979
65.000000 0.03941148500
66.000000 0.03855606332
67.000000 0.03828232511
68.000000 0.03537785808
69.000000 0.03606607696
70.000000 0.03255808083
71.000000 0.03427792490
72.000000 0.03000613821
73.000000 0.03247351617
74.000000 0.02903971802
75.000000 0.02878917215
76.000000 0.02846798141
77.000000 0.02776043678
78.000000 0.02602764493
79.000000 0.02726388465
80.000000 0.02622173876
81.000000 0.02470994308
82.000000 0.02474797951
83.000000 0.02627246005
84.000000 0.02316223055
85.000000 0.02422594932
86.000000 0.02403930661
87.000000 0.02266842862
88.000000 0.02261256047
89.000000 0.02358446115
90.000000 0.02256204758
91.000000 0.02256851786
92.000000 0.02285002969
93.000000 0.02154421587
94.000000 0.02333419005
95.000000 0.02126761532
96.000000 0.02235235562
97.000000 0.02124213329
98.000000 0.02166941266
99.000000 0.02246424166
100.000000 0.02142421363
101.000000 0.02251315169
102.000000 0.02468764544
103.000000 0.02340761037
104.000000 0.02620485669
105.000000 0.02933244902
106.000000 0.03026354494
107.000000 0.03191948518
108.000000 0.03105591357
109.000000 0.02701404595
110.000000 0.02257746451
111.000000 0.01626531665
112.000000 0.01234348208
113.000000 0.00735790210
114.000000 0.00538412788
115.000000 0.00316180982
116.000000 0.00195057046
117.000000 0.00143109799
118.000000 0.00113751659
119.000000 0.00102079247
120.000000 0.00105198888
121.000000 0.00102950979
122.000000 0.00090316992
123.000000 0.00064469207
124.000000 0.00051699786
125.000000 0.00043223325
126.000000 0.00050397957
127.000000 0.00042867949
128.000000 0.00033538028
129.000000 0.00031429579
130.000000 0.00026591973
131.000000 0.00026587914
132.000000 0.00020497667
133.000000 0.00017810869
134.000000 0.00018875096
135.000000 0.00019747290
136.000000 0.00014089363
137.000000 0.00014822881
138.000000 0.00020924223
139.000000 0.00017005176
140.000000 0.00012427904
141.000000 0.00011344647
142.000000 0.00011040113
143.000000 0.00009997024
144.000000 0.00016670845
145.000000 0.00010756004
146.000000 0.00008299270
147.000000 0.00008476062
148.000000 0.00014311963
149.000000 0.00007313488
150.000000 0.00011170749
151.000000 0.00007302000
152.000000 0.00007156976
153.000000 0.00008693304
154.000000 0.00005912891
155.000000 0.00009319862
156.000000 0.00004772542
157.000000 0.00008008732
158.000000 0.00004385304
159.000000 0.00007627489
160.000000 0.00003710464
161.000000 0.00006457627
162.000000 0.00003727886
163.000000 0.00005396591
164.000000 0.00003377372
165.000000 0.00004716603
166.000000 0.00003440441
167.000000 0.00004130484
168.000000 0.00003422794
169.000000 0.00003674775
170.000000 0.00003997164
171.000000 0.00003017929
172.000000 0.00004536065
173.000000 0.00002885263
174.000000 0.00004239683
175.000000 0.00002759974
176.000000 0.00004566803
177.000000 0.00002891492
178.000000 0.00004056563
179.000000 0.00003384600
180.000000 0.00003421829
181.000000 0.00004285623
182.000000 0.00002945352
183.000000 0.00004676932
184.000000 0.00003165147
185.000000 0.00004075823
186.000000 0.00003663333
187.000000 0.00003374257
188.000000 0.00004382426
189.000000 0.00002979663
190.000000 0.00004510974
191.000000 0.00003046999
192.000000 0.00003849094
193.000000 0.00003601631
194.000000 0.00003180164
195.000000 0.00004501979
196.000000 0.00003025138
197.000000 0.00003956530
198.000000 0.00003634932
199.000000 0.00003434410
200.000000 0.00004259758
201.000000 0.00003301666
202.000000 0.00004245038
203.000000 0.00003683826
204.000000 0.00003062925
205.000000 0.00004345883
206.000000 0.00002896932
207.000000 0.00003688539
208.000000 0.00003495910
209.000000 0.00002795539
210.000000 0.00003432804
211.000000 0.00002571217
212.000000 0.00003181315
213.000000 0.00003102656
214.000000 0.00002395840
215.000000 0.00003318400
216.000000 0.00002396080
217.000000 0.00002641970
218.000000 0.00002820339
219.000000 0.00002281636
220.000000 0.00002815902
221.000000 0.00002523799
222.000000 0.00002270187
223.000000 0.00003030904
224.000000 0.00002363682
225.000000 0.00002644830
226.000000 0.00003164072
227.000000 0.00002355166
228.000000 0.00003148572
229.000000 0.00002591609
230.000000 0.00002303570
231.000000 0.00002838774
232.000000 0.00002140430
233.000000 0.00002271755
234.000000 0.00002478245
235.000000 0.00001818477
236.000000 0.00002026793
237.000000 0.00002069000
238.000000 0.00001541706
239.000000 0.00001856154
240.000000 0.00001646341
241.000000 0.00001456142
242.000000 0.00001791943
243.000000 0.00001372979
244.000000 0.00001651498
245.000000 0.00001542232
246.000000 0.00001289483
247.000000 0.00001556535
248.000000 0.00001409286
249.000000 0.00001233234
250.000000 0.00001519824
251.000000 0.00001142356
252.000000 0.00001294690
253.000000 0.00001246149
254.000000 0.00001033178
255.000000 0.00001197638
256.000000 0.00001022704
257.000000 0.00001033203
258.000000 0.00001090633
259.000000 0.00000830885
260.000000 0.00000974493
261.000000 0.00000794466
262.000000 0.00000879087
263.000000 0.00000898412
264.000000 0.00000666785
265.000000 0.00000706362
266.000000 0.00000614724
267.000000 0.00000559193
268.000000 0.00000556118
269.000000 0.00000476319
270.000000 0.00000500582
271.000000 0.00000419342
272.000000 0.00000581873
273.000000 0.00000424136
274.000000 0.00000359291
275.000000 0.00000316572
276.000000 0.00000336390
277.000000 0.00000266197
278.000000 0.00000323425
279.000000 0.00000349069
280.000000 0.00000236454
281.000000 0.00000229281
282.000000 0.00000210621
283.000000 0.00000195385
284.000000 0.00000225603
285.000000 0.00000224226
286.000000 0.00000149977
287.000000 0.00000204432
288.000000 0.00000171284
289.000000 0.00000135187
290.000000 0.00000193806
291.000000 0.00000115443
292.000000 0.00000124687
293.000000 0.00000146777
294.000000 0.00000109758
295.000000 0.00000118645
296.000000 0.00000113345
297.000000 0.00000106686
298.000000 0.00000117385
299.000000 0.00000095445
300.000000 0.00000109038
301.000000 0.00000091022
302.000000 0.00000091199
303.000000 0.00000106405
304.000000 0.00000082000
305.000000 0.00000108958
306.000000 0.00000071290
307.000000 0.00000109637
308.000000 0.00000066814
309.000000 0.00000083771
310.000000 0.00000071362
311.000000 0.00000071199
312.000000 0.00000069100
313.000000 0.00000067439
314.000000 0.00000057037
315.000000 0.00000066184
316.000000 0.00000050680
317.000000 0.00000063065
318.000000 0.00000047404
319.000000 0.00000056326
320.000000 0.00000045621
321.000000 0.00000050946
322.000000 0.00000043238
323.000000 0.00000052090
324.000000 0.00000037851
325.000000 0.00000051914
326.000000 0.00000035160
327.000000 0.00000049116
328.000000 0.00000033848
329.000000 0.00000042353
330.000000 0.00000033666
331.000000 0.00000042217
332.000000 0.00000028234
333.000000 0.00000042871
334.000000 0.00000025984
335.000000 0.00000042912
336.000000 0.00000025750
337.000000 0.00000036169
338.000000 0.00000028441
339.000000 0.00000031904
340.000000 0.00000024526
341.000000 0.00000031931
342.000000 0.00000022676
343.000000 0.00000024048
344.000000 0.00000022305
345.000000 0.00000019749
346.000000 0.00000024242
347.000000 0.00000016659
348.000000 0.00000023846
349.000000 0.00000017169
350.000000 0.00000016540
351.000000 0.00000019016
352.000000 0.00000012441
353.000000 0.00000019189
354.000000 0.00000012246
355.000000 0.00000016643
356.000000 0.00000012104
357.000000 0.00000013634
358.000000 0.00000011679
359.000000 0.00000011812
360.000000 0.00000010988
361.000000 0.00000009708
362.000000 0.00000011474
363.000000 0.00000007629
364.000000 0.00000011169
365.000000 0.00000007658
366.000000 0.00000008726
367.000000 0.00000007415
368.000000 0.00000008216
369.000000 0.00000007622
370.000000 0.00000007070
371.000000 0.00000007788
372.000000 0.00000005657
373.000000 0.00000007482
374.000000 0.00000005382
375.000000 0.00000005911
376.000000 0.00000006857
377.000000 0.00000004033
378.000000 0.00000006272
379.000000 0.00000003818
380.000000 0.00000004812
381.000000 0.00000004313
382.000000 0.00000003620
383.000000 0.00000004422
384.000000 0.00000003604
385.000000 0.00000004101
386.000000 0.00000003468
387.000000 0.00000004298
388.000000 0.00000003146
389.000000 0.00000004460
390.000000 0.00000003771
391.000000 0.00000003509
392.000000 0.00000003894
393.000000 0.00000003355
394.000000 0.00000004357
395.000000 0.00000003518
396.000000 0.00000004683
397.000000 0.00000003839
398.000000 0.00000003331
399.000000 0.00000003954
400.000000 0.00000003088
401.000000 0.00000003708
402.000000 0.00000003012
403.000000 0.00000003684
404.000000 0.00000002614
405.000000 0.00000003558
406.000000 0.00000002226
407.000000 0.00000003362
408.000000 0.00000002386
409.000000 0.00000002021
410.000000 0.00000001709
411.000000 0.00000001881
412.000000 0.00000001472
413.000000 0.00000001641
414.000000 0.00000001342
415.000000 0.00000001610
416.000000 0.00000001559
417.000000 0.00000001755
418.000000 0.00000001257
419.000000 0.00000001720
420.000000 0.00000001720
421.000000 0.00000001138
422.000000 0.00000001635
423.000000 0.00000001189
424.000000 0.00000001264
425.000000 0.00000001366
426.000000 0.00000001259
427.000000 0.00000001078
428.000000 0.00000001383
429.000000 0.00000001251
430.000000 0.00000001014
431.000000 0.00000001511
432.000000 0.00000001028
433.000000 0.00000001150
434.000000 0.00000001167
435.000000 0.00000000988
436.000000 0.00000000984
437.000000 0.00000000892
438.000000 0.00000000928
439.000000 0.00000000939
440.000000 0.00000000786
441.000000 0.00000000716
442.000000 0.00000000838
443.000000 0.00000000702
444.000000 0.00000000550
445.000000 0.00000000775
446.000000 0.00000000471
447.000000 0.00000000578
448.000000 0.00000000506
449.000000 0.00000000377
450.000000 0.00000000498
451.000000 0.00000000344
452.000000 0.00000000374
453.000000 0.00000000319
454.000000 0.00000000309
455.000000 0.00000000288
456.000000 0.00000000306
457.000000 0.00000000210
458.000000 0.00000000319
459.000000 0.00000000172
460.000000 0.00000000255
461.000000 0.00000000181
462.000000 0.00000000200
463.000000 0.00000000185
464.000000 0.00000000183
465.000000 0.00000000150
466.000000 0.00000000175
467.000000 0.00000000129
468.000000 0.00000000199
469.000000 0.00000000117
470.000000 0.00000000129
471.000000 0.00000000144
472.000000 0.00000000101
473.000000 0.00000000126
474.000000 0.00000000097
475.000000 0.00000000098
476.000000 0.00000000097
477.000000 0.00000000095
478.000000 0.00000000074
479.000000 0.00000000107
480.000000 0.00000000069
481.000000 0.00000000107
482.000000 0.00000000060
483.000000 0.00000000083
484.000000 0.00000000058
485.000000 0.00000000067
486.000000 0.00000000056
487.000000 0.00000000063
488.000000 0.00000000045
489.000000 0.00000000058
490.000000 0.00000000037
491.000000 0.00000000052
492.000000 0.00000000029
493.000000 0.00000000041
494.000000 0.00000000027
495.000000 0.00000000032
496.000000 0.00000000028
497.000000 0.00000000026
498.000000 0.00000000024
499.000000 0.00000000028
500.000000 0.00000000018
501.000000 0.00000000027
502.000000 0.00000000016
503.000000 0.00000000023
504.000000 0.00000000017
505.000000 0.00000000016
506.000000 0.00000000018
507.000000 0.00000000014
508.000000 0.00000000016
509.000000 0.00000000014
510.000000 0.00000000014
511.000000 0.00000000013
512.000000 0.00000000014
513.000000 0.00000000009


==> data/CG_alone_D10000.tex <==
0.000000 1.00000000000
1.000000 0.51769507923
2.000000 2.51939916083
3.000000 0.51464443985
4.000000 0.56943475096
5.000000 1.45177875458
6.000000 1.24255602337
7.000000 0.64072330819
8.000000 0.48861699731
9.000000 0.57047021286
10.000000 0.89397597405
11.000000 0.95645120023
12.000000 0.87786547343
13.000000 0.67185877228
14.000000 0.51470959937
15.000000 0.43315039672
16.000000 0.58629312230
17.000000 0.69034237400
18.000000 0.78037100779
19.000000 0.78603884151
20.000000 0.60527673780
21.000000 0.46976261958
22.000000 0.40287165247
23.000000 0.49462996146
24.000000 0.55839348855
25.000000 0.62111814655
26.000000 0.64699089451
27.000000 0.61928669745
28.000000 0.49963494902
29.000000 0.47121149120
30.000000 0.44891213978
31.000000 0.42092503166
32.000000 0.48117248995
33.000000 0.50027459610
34.000000 0.56549455193
35.000000 0.56023158417
36.000000 0.52730827111
37.000000 0.46385161916
38.000000 0.39525769446
39.000000 0.40447960606
40.000000 0.44372034839
41.000000 0.47280262623
42.000000 0.49572542179
43.000000 0.51812110642
44.000000 0.46897557607
45.000000 0.42755040507
46.000000 0.39547025738
47.000000 0.40020553645
48.000000 0.41153705426
49.000000 0.43005285698
50.000000 0.47044496427
51.000000 0.45515181492
52.000000 0.44701698924
53.000000 0.42776118877
54.000000 0.38221561155
55.000000 0.35737495365
56.000000 0.36713887988
57.000000 0.42643896079
58.000000 0.40135685599
59.000000 0.46443916943
60.000000 0.41937091951
61.000000 0.41043377768
62.000000 0.35968031626
63.000000 0.34284352963
64.000000 0.33264342305
65.000000 0.36594815982
66.000000 0.38055339224
67.000000 0.37124401184
68.000000 0.48635707113
69.000000 0.38239119799
70.000000 0.33022349248
71.000000 0.31581293975
72.000000 0.31884566241
73.000000 0.36830303778
74.000000 0.31848302880
75.000000 0.31607898524
76.000000 0.38601132726
77.000000 0.37292441109
78.000000 0.36256994120
79.000000 0.31807136231
80.000000 0.33082384461
81.000000 0.29312743143
82.000000 0.28150370071
83.000000 0.29920604788
84.000000 0.30295698527
85.000000 0.32983445709
86.000000 0.33280347110
87.000000 0.34877322752
88.000000 0.31401140471
89.000000 0.28046575190
90.000000 0.24342419783
91.000000 0.29015762206
92.000000 0.27141661952
93.000000 0.25510920732
94.000000 0.28466580109
95.000000 0.32982823470
96.000000 0.31171707664
97.000000 0.24042589088
98.000000 0.25188390691
99.000000 0.24857691752
100.000000 0.27690737611
101.000000 0.23055054750
102.000000 0.22788504518
103.000000 0.24150624883
104.000000 0.26166186439
105.000000 0.24929370458
106.000000 0.26233761414
107.000000 0.25326628721
108.000000 0.21121025582
109.000000 0.23081199358
110.000000 0.20232383301
111.000000 0.20142559026
112.000000 0.20604008090
113.000000 0.21612713172
114.000000 0.27173807416
115.000000 0.19728173135
116.000000 0.18979037435
117.000000 0.16660712047
118.000000 0.14236158648
119.000000 0.16229858970
120.000000 0.16199128567
121.000000 0.17092392608
122.000000 0.12943209735
123.000000 0.15093546724
124.000000 0.12833956565
125.000000 0.11886633288
126.000000 0.11429924301
127.000000 0.16150343290
128.000000 0.14304781305
129.000000 0.08448108101
130.000000 0.10765984051
131.000000 0.09906875106
132.000000 0.17197606321
133.000000 0.08515318310
134.000000 0.20280921533
135.000000 0.08258782103
136.000000 0.18630628043
137.000000 0.08803781894
138.000000 0.12718505912
139.000000 0.13943278943
140.000000 0.06914493914
141.000000 0.15669878330
142.000000 0.07054179474
143.000000 0.20937351100
144.000000 0.10229586918
145.000000 0.05890500977
146.000000 0.16081163613
147.000000 0.09620636658
148.000000 0.06898761453
149.000000 0.19264695549
150.000000 0.06958634352
151.000000 0.06256188882
152.000000 0.16002389787
153.000000 0.07913589520
154.000000 0.05983816322
155.000000 0.12595393793
156.000000 0.12563485583
157.000000 0.04851297908
158.000000 0.06752500295
159.000000 0.14230603652
160.000000 0.08290802215
161.000000 0.04861028248
162.000000 0.10245786322
163.000000 0.09945389946
164.000000 0.05469345763
165.000000 0.05725805265
166.000000 0.11383683886
167.000000 0.08587563548
168.000000 0.04358615603
169.000000 0.05471770006
170.000000 0.13115816030
171.000000 0.07628152458
172.000000 0.03879349400
173.000000 0.04690106250
174.000000 0.09380790644
175.000000 0.10189557512
176.000000 0.05870372379
177.000000 0.03468866931
178.000000 0.05177796015
179.000000 0.09586003819
180.000000 0.08099997469
181.000000 0.04458217839
182.000000 0.03685594244
183.000000 0.06175419212
184.000000 0.08710839987
185.000000 0.05417221262
186.000000 0.03391460999
187.000000 0.04701313015
188.000000 0.08121443092
189.000000 0.07471988536
190.000000 0.04188366649
191.000000 0.03360542218
192.000000 0.04422100431
193.000000 0.06973064401
194.000000 0.07870042803
195.000000 0.03487459394
196.000000 0.03359187847
197.000000 0.05214870120
198.000000 0.06766704195
199.000000 0.06320547642
200.000000 0.03514317218
201.000000 0.03327746473
202.000000 0.04636885267
203.000000 0.05908518639
204.000000 0.06909303564
205.000000 0.04398134098
206.000000 0.02769213680
207.000000 0.03333165226
208.000000 0.05328305968
209.000000 0.07364793903
210.000000 0.05378116567
211.000000 0.02982776116
212.000000 0.02760747703
213.000000 0.03798105437
214.000000 0.06252590200
215.000000 0.06035965735
216.000000 0.04713547282
217.000000 0.03179863952
218.000000 0.02792233609
219.000000 0.03271010881
220.000000 0.05313647307
221.000000 0.07015188283
222.000000 0.04040627430
223.000000 0.02645363266
224.000000 0.02696414189
225.000000 0.04408806378
226.000000 0.05665666585
227.000000 0.05050863364
228.000000 0.03788805886
229.000000 0.03026521289
230.000000 0.03120633320
231.000000 0.03691412678
232.000000 0.04730048732
233.000000 0.05301380632
234.000000 0.02971471138
235.000000 0.02593695608
236.000000 0.03249121174
237.000000 0.05035981889
238.000000 0.03460245002
239.000000 0.02688785869
240.000000 0.02618162837
241.000000 0.03499952734
242.000000 0.04735250609
243.000000 0.05355457886
244.000000 0.02475071269
245.000000 0.02283208938
246.000000 0.03770424922
247.000000 0.04355816612
248.000000 0.02529138667
249.000000 0.02483249506
250.000000 0.03866915166
251.000000 0.03285975846
252.000000 0.03309644684
253.000000 0.03570862247
254.000000 0.02922231426
255.000000 0.02601245204
256.000000 0.07476762758
257.000000 0.05059217600
258.000000 0.03800307134
259.000000 0.03066106486
260.000000 0.03293846002
261.000000 0.05540102411
262.000000 0.05817919088
263.000000 0.06831283763
264.000000 0.04626682026
265.000000 0.03363365036
266.000000 0.04186386198
267.000000 0.06171843012
268.000000 0.05388649451
269.000000 0.07999506543
270.000000 0.03004943051
271.000000 0.04030530669
272.000000 0.03078762372
273.000000 0.04929423868
274.000000 0.04281648091
275.000000 0.01949138062
276.000000 0.02651532704
277.000000 0.01305864774
278.000000 0.01627467973
279.000000 0.01760661912
280.000000 0.01597073454
281.000000 0.01256731236
282.000000 0.00508380930
283.000000 0.00823115371
284.000000 0.00374645665
285.000000 0.00476919049
286.000000 0.00684201295
287.000000 0.00235671267
288.000000 0.00259202019
289.000000 0.00203976291
290.000000 0.00132394670
291.000000 0.00261741383
292.000000 0.00193953867
293.000000 0.00153966108
294.000000 0.00224710354
295.000000 0.00096397507
296.000000 0.00132826423
297.000000 0.00153654623
298.000000 0.00109681304
299.000000 0.00180164011
300.000000 0.00204619870
301.000000 0.00078823978
302.000000 0.00103797123
303.000000 0.00091923533
304.000000 0.00061004802
305.000000 0.00103788824
306.000000 0.00117557400
307.000000 0.00051928200
308.000000 0.00055296032
309.000000 0.00066873729
310.000000 0.00044544657
311.000000 0.00044804362
312.000000 0.00101159814
313.000000 0.00068701407
314.000000 0.00041347782
315.000000 0.00054841696
316.000000 0.00057420251
317.000000 0.00036875075
318.000000 0.00048404589
319.000000 0.00080739949
320.000000 0.00042438702
321.000000 0.00026389825
322.000000 0.00042995459
323.000000 0.00041610739
324.000000 0.00027760816
325.000000 0.00050488752
326.000000 0.00069432330
327.000000 0.00037894913
328.000000 0.00024649865
329.000000 0.00033743055
330.000000 0.00046800965
331.000000 0.00031822236
332.000000 0.00031846512
333.000000 0.00050763491
334.000000 0.00033439772
335.000000 0.00019088361
336.000000 0.00022020346
337.000000 0.00040936638
338.000000 0.00040042312
339.000000 0.00025702247
340.000000 0.00036923679
341.000000 0.00035522718
342.000000 0.00023401511
343.000000 0.00017999431
344.000000 0.00030499437
345.000000 0.00040338089
346.000000 0.00019906382
347.000000 0.00020638103
348.000000 0.00030980372
349.000000 0.00020235124
350.000000 0.00014779721
351.000000 0.00023697809
352.000000 0.00036252504
353.000000 0.00019697052
354.000000 0.00011281538
355.000000 0.00021417524
356.000000 0.00031823061
357.000000 0.00029268694
358.000000 0.00013047533
359.000000 0.00011325206
360.000000 0.00022390892
361.000000 0.00020847098
362.000000 0.00013706359
363.000000 0.00018084018
364.000000 0.00020438737
365.000000 0.00009267959
366.000000 0.00015547632
367.000000 0.00020880158
368.000000 0.00020469854
369.000000 0.00009402551
370.000000 0.00016577332
371.000000 0.00018041380
372.000000 0.00012665854
373.000000 0.00012746122
374.000000 0.00021478843
375.000000 0.00021851275
376.000000 0.00009394370
377.000000 0.00008326364
378.000000 0.00017147638
379.000000 0.00019302538
380.000000 0.00018841070
381.000000 0.00008554564
382.000000 0.00010833711
383.000000 0.00018085751
384.000000 0.00014945722
385.000000 0.00011573801
386.000000 0.00010478506
387.000000 0.00015742260
388.000000 0.00010837085
389.000000 0.00010330072
390.000000 0.00009087571
391.000000 0.00017598448
392.000000 0.00018627929
393.000000 0.00006774086
394.000000 0.00010361374
395.000000 0.00008063973
396.000000 0.00016730223
397.000000 0.00010143422
398.000000 0.00010854666
399.000000 0.00005513646
400.000000 0.00014991070
401.000000 0.00008311096
402.000000 0.00009495567
403.000000 0.00006000603
404.000000 0.00011668547
405.000000 0.00007629861
406.000000 0.00010259134
407.000000 0.00004336828
408.000000 0.00005000496
409.000000 0.00007659357
410.000000 0.00008413590
411.000000 0.00008480138
412.000000 0.00003196604
413.000000 0.00005540577
414.000000 0.00007250623
415.000000 0.00006548120
416.000000 0.00005468419
417.000000 0.00002676774
418.000000 0.00005565140
419.000000 0.00004475051
420.000000 0.00006005517
421.000000 0.00003690417
422.000000 0.00003183421
423.000000 0.00005503441
424.000000 0.00004336640
425.000000 0.00004630993
426.000000 0.00002854269
427.000000 0.00002041730
428.000000 0.00004640723
429.000000 0.00003328717
430.000000 0.00005205442
431.000000 0.00002324155
432.000000 0.00001925927
433.000000 0.00003023820
434.000000 0.00002829017
435.000000 0.00003775687
436.000000 0.00003926191
437.000000 0.00001462212
438.000000 0.00002148978
439.000000 0.00003000797
440.000000 0.00002545886
441.000000 0.00003156681
442.000000 0.00001982455
443.000000 0.00001792406
444.000000 0.00003435879
445.000000 0.00001906306
446.000000 0.00002239807
447.000000 0.00001530934
448.000000 0.00001320913
449.000000 0.00003295094
450.000000 0.00002719317
451.000000 0.00001844946
452.000000 0.00001941490
453.000000 0.00001247941
454.000000 0.00001446840
455.000000 0.00002987645
456.000000 0.00002652018
457.000000 0.00001231470
458.000000 0.00001578738
459.000000 0.00001359041
460.000000 0.00001708925
461.000000 0.00002969942
462.000000 0.00002232359
463.000000 0.00001221967
464.000000 0.00001770471
465.000000 0.00001347193
466.000000 0.00001329935
467.000000 0.00002949074
468.000000 0.00001712750
469.000000 0.00001205107
470.000000 0.00001226495
471.000000 0.00002058433
472.000000 0.00001721718
473.000000 0.00001931084
474.000000 0.00001649783
475.000000 0.00000949359
476.000000 0.00001324203
477.000000 0.00002097100
478.000000 0.00001825661
479.000000 0.00001732852
480.000000 0.00001868768
481.000000 0.00001208890
482.000000 0.00000872775
483.000000 0.00002416267
484.000000 0.00000922552
485.000000 0.00001284432
486.000000 0.00002092966
487.000000 0.00001271134
488.000000 0.00001291045
489.000000 0.00001164376
490.000000 0.00001024859
491.000000 0.00001789455
492.000000 0.00002352836
493.000000 0.00001237819
494.000000 0.00000734805
495.000000 0.00001579283
496.000000 0.00001689760
497.000000 0.00001338987
498.000000 0.00001601033
499.000000 0.00001239230
500.000000 0.00000749881
501.000000 0.00001077100
502.000000 0.00002662352
503.000000 0.00000970392
504.000000 0.00001113494
505.000000 0.00000888449
506.000000 0.00001371108
507.000000 0.00001072451
508.000000 0.00001643680
509.000000 0.00001878588
510.000000 0.00000739457
511.000000 0.00001031508
512.000000 0.00001073092
513.000000 0.00001856000
514.000000 0.00001087207
515.000000 0.00000955145
516.000000 0.00001760729
517.000000 0.00000862438
518.000000 0.00001121372
519.000000 0.00001490045
520.000000 0.00001039291
521.000000 0.00000999915
522.000000 0.00001004578
523.000000 0.00002375854
524.000000 0.00001087350
525.000000 0.00001159634
526.000000 0.00000915980
527.000000 0.00001728567
528.000000 0.00000995238
529.000000 0.00001351082
530.000000 0.00001751721
531.000000 0.00001320810
532.000000 0.00000718909
533.000000 0.00001303313
534.000000 0.00001661953
535.000000 0.00001693539
536.000000 0.00001020695
537.000000 0.00001766674
538.000000 0.00001043267
539.000000 0.00001193528
540.000000 0.00000816513
541.000000 0.00002277764
542.000000 0.00001740391
543.000000 0.00000915481
544.000000 0.00001001513
545.000000 0.00000842750
546.000000 0.00001853974
547.000000 0.00000931418
548.000000 0.00001643166
549.000000 0.00001343634
550.000000 0.00001682410
551.000000 0.00000642402
552.000000 0.00000810459
553.000000 0.00001879965
554.000000 0.00001439629
555.000000 0.00001113419
556.000000 0.00000789370
557.000000 0.00001200571
558.000000 0.00001119086
559.000000 0.00001090485
560.000000 0.00001135363
561.000000 0.00001205750
562.000000 0.00001617195
563.000000 0.00000714316
564.000000 0.00001230713
565.000000 0.00001202134
566.000000 0.00001509437
567.000000 0.00001483060
568.000000 0.00000669770
569.000000 0.00001036001
570.000000 0.00001557048
571.000000 0.00001421848
572.000000 0.00001233842
573.000000 0.00000616046
574.000000 0.00000896751
575.000000 0.00001638216
576.000000 0.00001407854
577.000000 0.00001534169
578.000000 0.00000891194
579.000000 0.00000635387
580.000000 0.00001436045
581.000000 0.00001069988
582.000000 0.00001635912
583.000000 0.00000946520
584.000000 0.00000979844
585.000000 0.00001460291
586.000000 0.00000854276
587.000000 0.00001005445
588.000000 0.00000790868
589.000000 0.00001237718
590.000000 0.00001234292
591.000000 0.00000799371
592.000000 0.00000897800
593.000000 0.00000916078
594.000000 0.00001241183
595.000000 0.00001789668
596.000000 0.00000827704
597.000000 0.00000803257
598.000000 0.00001199492
599.000000 0.00001216253
600.000000 0.00001871649
601.000000 0.00001533061
602.000000 0.00000893754
603.000000 0.00001242878
604.000000 0.00000951406
605.000000 0.00000769190
606.000000 0.00001209183
607.000000 0.00001592758
608.000000 0.00001894100
609.000000 0.00000843586
610.000000 0.00000572540
611.000000 0.00001693152
612.000000 0.00001451387
613.000000 0.00000811230
614.000000 0.00000560457
615.000000 0.00001156641
616.000000 0.00001197574
617.000000 0.00001393263
618.000000 0.00001117845
619.000000 0.00000586406
620.000000 0.00000796483
621.000000 0.00001406606
622.000000 0.00000731229
623.000000 0.00000839904
624.000000 0.00001365140
625.000000 0.00000735161
626.000000 0.00001269604
627.000000 0.00000600259
628.000000 0.00000582728
629.000000 0.00001351523
630.000000 0.00000893111
631.000000 0.00000791461
632.000000 0.00000719316
633.000000 0.00000609831
634.000000 0.00000654483
635.000000 0.00000815038
636.000000 0.00000784538
637.000000 0.00000528956
638.000000 0.00000908847
639.000000 0.00000731995
640.000000 0.00000621892
641.000000 0.00001034560
642.000000 0.00000448478
643.000000 0.00001071389
644.000000 0.00000766989
645.000000 0.00000445994
646.000000 0.00000611720
647.000000 0.00000822958
648.000000 0.00000639536
649.000000 0.00000448982
650.000000 0.00000569983
651.000000 0.00000527741
652.000000 0.00000558043
653.000000 0.00000933579
654.000000 0.00000722265
655.000000 0.00000477032
656.000000 0.00000312535
657.000000 0.00000821855
658.000000 0.00000611191
659.000000 0.00000658276
660.000000 0.00000529641
661.000000 0.00000388566
662.000000 0.00000380955
663.000000 0.00000846637
664.000000 0.00000633547
665.000000 0.00000289744
666.000000 0.00000525033
667.000000 0.00000562496
668.000000 0.00000931268
669.000000 0.00000542020
670.000000 0.00000556071
671.000000 0.00000440237
672.000000 0.00000410397
673.000000 0.00000431633
674.000000 0.00000882113
675.000000 0.00000568085
676.000000 0.00000512581
677.000000 0.00000400101
678.000000 0.00000776145
679.000000 0.00000452057
680.000000 0.00000423750
681.000000 0.00000385706
682.000000 0.00000803948
683.000000 0.00000513174
684.000000 0.00000586847
685.000000 0.00000549528
686.000000 0.00000426976
687.000000 0.00000341643
688.000000 0.00000333365
689.000000 0.00001009856
690.000000 0.00000302448
691.000000 0.00000266175
692.000000 0.00000446420
693.000000 0.00000578539
694.000000 0.00000580990
695.000000 0.00000336340
696.000000 0.00000466576
697.000000 0.00000305866
698.000000 0.00000294622
699.000000 0.00000452369
700.000000 0.00000520838
701.000000 0.00000597709
702.000000 0.00000255608
703.000000 0.00000240833
704.000000 0.00000461336
705.000000 0.00000496396
706.000000 0.00000570999
707.000000 0.00000295768
708.000000 0.00000385987
709.000000 0.00000351017
710.000000 0.00000211538
711.000000 0.00000415015
712.000000 0.00000416218
713.000000 0.00000600105
714.000000 0.00000175286
715.000000 0.00000294383
716.000000 0.00000397796
717.000000 0.00000253629
718.000000 0.00000282147
719.000000 0.00000240252
720.000000 0.00000498963
721.000000 0.00000204140
722.000000 0.00000171591
723.000000 0.00000290439
724.000000 0.00000285563
725.000000 0.00000371456
726.000000 0.00000171386
727.000000 0.00000259662
728.000000 0.00000288250
729.000000 0.00000171229
730.000000 0.00000244636
731.000000 0.00000252641
732.000000 0.00000299224
733.000000 0.00000166480
734.000000 0.00000152153
735.000000 0.00000283093
736.000000 0.00000207679
737.000000 0.00000204652
738.000000 0.00000195719
739.000000 0.00000194921
740.000000 0.00000317662
741.000000 0.00000201218
742.000000 0.00000117441
743.000000 0.00000220066
744.000000 0.00000193816
745.000000 0.00000218678
746.000000 0.00000218790
747.000000 0.00000170527
748.000000 0.00000231625
749.000000 0.00000114565
750.000000 0.00000128510
751.000000 0.00000331577
752.000000 0.00000225178
753.000000 0.00000199946
754.000000 0.00000148096
755.000000 0.00000113464
756.000000 0.00000146699
757.000000 0.00000243406
758.000000 0.00000203076
759.000000 0.00000157341
760.000000 0.00000143073
761.000000 0.00000138077
762.000000 0.00000164273
763.000000 0.00000144233
764.000000 0.00000179471
765.000000 0.00000164893
766.000000 0.00000128884
767.000000 0.00000141866
768.000000 0.00000102980
769.000000 0.00000135461
770.000000 0.00000192044
771.000000 0.00000165167
772.000000 0.00000084754
773.000000 0.00000109208
774.000000 0.00000133431
775.000000 0.00000178471
776.000000 0.00000094496
777.000000 0.00000179808
778.000000 0.00000119209
779.000000 0.00000082622
780.000000 0.00000118851
781.000000 0.00000189940
782.000000 0.00000148006
783.000000 0.00000078973
784.000000 0.00000156132
785.000000 0.00000103695
786.000000 0.00000091517
787.000000 0.00000107908
788.000000 0.00000241158
789.000000 0.00000075102
790.000000 0.00000073750
791.000000 0.00000119412
792.000000 0.00000134061
793.000000 0.00000116894
794.000000 0.00000145122
795.000000 0.00000077915
796.000000 0.00000069162
797.000000 0.00000112145
798.000000 0.00000151595
799.000000 0.00000100666
800.000000 0.00000071856
801.000000 0.00000072128
802.000000 0.00000091752
803.000000 0.00000089675
804.000000 0.00000179117
805.000000 0.00000056762
806.000000 0.00000055489
807.000000 0.00000100676
808.000000 0.00000129288
809.000000 0.00000052327
810.000000 0.00000089719
811.000000 0.00000088139
812.000000 0.00000075075
813.000000 0.00000118293
814.000000 0.00000053681
815.000000 0.00000052230
816.000000 0.00000122028
817.000000 0.00000103805
818.000000 0.00000088198
819.000000 0.00000063405
820.000000 0.00000094637
821.000000 0.00000071643
822.000000 0.00000073578
823.000000 0.00000071328
824.000000 0.00000100734
825.000000 0.00000066836
826.000000 0.00000118826
827.000000 0.00000083657
828.000000 0.00000054697
829.000000 0.00000048970
830.000000 0.00000106937
831.000000 0.00000119782
832.000000 0.00000080152
833.000000 0.00000048284
834.000000 0.00000061083
835.000000 0.00000096379
836.000000 0.00000078114
837.000000 0.00000093949
838.000000 0.00000096821
839.000000 0.00000088308
840.000000 0.00000047565
841.000000 0.00000074234
842.000000 0.00000099993
843.000000 0.00000053045
844.000000 0.00000098447
845.000000 0.00000065391
846.000000 0.00000062348
847.000000 0.00000048690
848.000000 0.00000049965
849.000000 0.00000068795
850.000000 0.00000086014
851.000000 0.00000037796
852.000000 0.00000038404
853.000000 0.00000090656
854.000000 0.00000086106
855.000000 0.00000051038
856.000000 0.00000034907
857.000000 0.00000055410
858.000000 0.00000067327
859.000000 0.00000101342
860.000000 0.00000039682
861.000000 0.00000035158
862.000000 0.00000063431
863.000000 0.00000050100
864.000000 0.00000060779
865.000000 0.00000089502
866.000000 0.00000051097
867.000000 0.00000045024
868.000000 0.00000038347
869.000000 0.00000051469
870.000000 0.00000058263
871.000000 0.00000039040
872.000000 0.00000066576
873.000000 0.00000068910
874.000000 0.00000046049
875.000000 0.00000042209
876.000000 0.00000037679
877.000000 0.00000055841
878.000000 0.00000066173
879.000000 0.00000049367
880.000000 0.00000077850
881.000000 0.00000056774
882.000000 0.00000022087
883.000000 0.00000071196
884.000000 0.00000066706
885.000000 0.00000053812
886.000000 0.00000051909
887.000000 0.00000024013
888.000000 0.00000065091
889.000000 0.00000061433
890.000000 0.00000032095
891.000000 0.00000056655
892.000000 0.00000042688
893.000000 0.00000052975
894.000000 0.00000047796
895.000000 0.00000022319
896.000000 0.00000057285
897.000000 0.00000036734
898.000000 0.00000038325
899.000000 0.00000055625
900.000000 0.00000026270
901.000000 0.00000027637
902.000000 0.00000030395
903.000000 0.00000036817
904.000000 0.00000051599
905.000000 0.00000027775
906.000000 0.00000021703
907.000000 0.00000027380
908.000000 0.00000053482
909.000000 0.00000022475
910.000000 0.00000016037
911.000000 0.00000048823
912.000000 0.00000023313
913.000000 0.00000037330
914.000000 0.00000016936
915.000000 0.00000028970
916.000000 0.00000020207
917.000000 0.00000026470
918.000000 0.00000037926
919.000000 0.00000024911
920.000000 0.00000013580
921.000000 0.00000019294
922.000000 0.00000022124
923.000000 0.00000030581
924.000000 0.00000034702
925.000000 0.00000023525
926.000000 0.00000011193
927.000000 0.00000022583
928.000000 0.00000023298
929.000000 0.00000033130
930.000000 0.00000025068
931.000000 0.00000019425
932.000000 0.00000010869
933.000000 0.00000027557
934.000000 0.00000018852
935.000000 0.00000024764
936.000000 0.00000014839
937.000000 0.00000012790
938.000000 0.00000018085
939.000000 0.00000024037
940.000000 0.00000013735
941.000000 0.00000017476
942.000000 0.00000019270
943.000000 0.00000014815
944.000000 0.00000014199
945.000000 0.00000015793
946.000000 0.00000019426
947.000000 0.00000020810
948.000000 0.00000018791
949.000000 0.00000011706
950.000000 0.00000009012
951.000000 0.00000032251
952.000000 0.00000011190
953.000000 0.00000008401
954.000000 0.00000017513
955.000000 0.00000024193
956.000000 0.00000016390
957.000000 0.00000011608
958.000000 0.00000018144
959.000000 0.00000007440
960.000000 0.00000012235
961.000000 0.00000023940
962.000000 0.00000009742
963.000000 0.00000009294
964.000000 0.00000011168
965.000000 0.00000012322
966.000000 0.00000012919
967.000000 0.00000019783
968.000000 0.00000009235
969.000000 0.00000008149
970.000000 0.00000011152
971.000000 0.00000012263
972.000000 0.00000008759
973.000000 0.00000010594
974.000000 0.00000015061
975.000000 0.00000008840
976.000000 0.00000006783
977.000000 0.00000009607
978.000000 0.00000012350
979.000000 0.00000008730
980.000000 0.00000008721
981.000000 0.00000009677
982.000000 0.00000013663
983.000000 0.00000005701
984.000000 0.00000011199
985.000000 0.00000008602
986.000000 0.00000010345
987.000000 0.00000006683
988.000000 0.00000008830
989.000000 0.00000006620
990.000000 0.00000010796
991.000000 0.00000005074
992.000000 0.00000007440
993.000000 0.00000012085
994.000000 0.00000006796
995.000000 0.00000009615
996.000000 0.00000005608
997.000000 0.00000004337
998.000000 0.00000012135
999.000000 0.00000011359
1000.000000 0.00000005554
1001.000000 0.00000006428
1002.000000 0.00000005244
1003.000000 0.00000006941
1004.000000 0.00000006283
1005.000000 0.00000008675
1006.000000 0.00000007802
1007.000000 0.00000006902
1008.000000 0.00000007599
1009.000000 0.00000005095
1010.000000 0.00000005358
1011.000000 0.00000007565
1012.000000 0.00000007948
1013.000000 0.00000010917
1014.000000 0.00000005923
1015.000000 0.00000003673
1016.000000 0.00000010948
1017.000000 0.00000007734
1018.000000 0.00000007034
1019.000000 0.00000004558
1020.000000 0.00000008237
1021.000000 0.00000010311
1022.000000 0.00000003490
1023.000000 0.00000005745
1024.000000 0.00000005267
1025.000000 0.00000007399
1026.000000 0.00000007824
1027.000000 0.00000005639
1028.000000 0.00000005356
1029.000000 0.00000002787
1030.000000 0.00000004527
1031.000000 0.00000008591
1032.000000 0.00000003806
1033.000000 0.00000003650
1034.000000 0.00000004221
1035.000000 0.00000003057
1036.000000 0.00000004677
1037.000000 0.00000005012
1038.000000 0.00000005010
1039.000000 0.00000003648
1040.000000 0.00000002631
1041.000000 0.00000005276
1042.000000 0.00000004112
1043.000000 0.00000003099
1044.000000 0.00000002224
1045.000000 0.00000006592
1046.000000 0.00000003205
1047.000000 0.00000003116
1048.000000 0.00000001715
1049.000000 0.00000002862
1050.000000 0.00000005722
1051.000000 0.00000002299
1052.000000 0.00000001939
1053.000000 0.00000002487
1054.000000 0.00000002331
1055.000000 0.00000003768
1056.000000 0.00000003324
1057.000000 0.00000001769
1058.000000 0.00000003999
1059.000000 0.00000002069
1060.000000 0.00000001681
1061.000000 0.00000002450
1062.000000 0.00000002214
1063.000000 0.00000002367
1064.000000 0.00000003049
1065.000000 0.00000002105
1066.000000 0.00000002734
1067.000000 0.00000001172
1068.000000 0.00000001488
1069.000000 0.00000003920
1070.000000 0.00000001242
1071.000000 0.00000001703
1072.000000 0.00000001580
1073.000000 0.00000001510
1074.000000 0.00000001835
1075.000000 0.00000002152
1076.000000 0.00000001034
1077.000000 0.00000001841
1078.000000 0.00000001984
1079.000000 0.00000001917
1080.000000 0.00000001272
1081.000000 0.00000001734
1082.000000 0.00000001491
1083.000000 0.00000001714
1084.000000 0.00000001155
1085.000000 0.00000001269
1086.000000 0.00000001331
1087.000000 0.00000002482
1088.000000 0.00000000914
1089.000000 0.00000001016
1090.000000 0.00000000912
1091.000000 0.00000001780
1092.000000 0.00000001820
1093.000000 0.00000001678
1094.000000 0.00000000625
1095.000000 0.00000001107
1096.000000 0.00000001883
1097.000000 0.00000001238
1098.000000 0.00000001791
1099.000000 0.00000001079
1100.000000 0.00000000949
1101.000000 0.00000001126
1102.000000 0.00000000970
1103.000000 0.00000001738
1104.000000 0.00000001557
1105.000000 0.00000001295
1106.000000 0.00000000720
1107.000000 0.00000001199
1108.000000 0.00000001265
1109.000000 0.00000001628
1110.000000 0.00000000782
1111.000000 0.00000000761
1112.000000 0.00000001653
1113.000000 0.00000002354
1114.000000 0.00000000900
1115.000000 0.00000001164
1116.000000 0.00000001030
1117.000000 0.00000000892
1118.000000 0.00000001556
1119.000000 0.00000001360
1120.000000 0.00000001274
1121.000000 0.00000001145
1122.000000 0.00000001003
1123.000000 0.00000000817
1124.000000 0.00000001549
1125.000000 0.00000001306
1126.000000 0.00000001316
1127.000000 0.00000000812
1128.000000 0.00000001860
1129.000000 0.00000001162
1130.000000 0.00000000635
1131.000000 0.00000001135
1132.000000 0.00000001715
1133.000000 0.00000001404
1134.000000 0.00000000673
1135.000000 0.00000000596
1136.000000 0.00000001476
1137.000000 0.00000001247
1138.000000 0.00000000975
1139.000000 0.00000000568
1140.000000 0.00000000998
1141.000000 0.00000001272
1142.000000 0.00000000744
1143.000000 0.00000000786
1144.000000 0.00000000624
1145.000000 0.00000000906
1146.000000 0.00000001159
1147.000000 0.00000000592
1148.000000 0.00000000516
1149.000000 0.00000000781
1150.000000 0.00000001146
1151.000000 0.00000000511
1152.000000 0.00000001066
1153.000000 0.00000000695
1154.000000 0.00000000680
1155.000000 0.00000000431
1156.000000 0.00000000784
1157.000000 0.00000000787
1158.000000 0.00000000411
1159.000000 0.00000000875
1160.000000 0.00000000692
1161.000000 0.00000000647
1162.000000 0.00000000325
1163.000000 0.00000000464
1164.000000 0.00000000644
1165.000000 0.00000000566
1166.000000 0.00000000859
1167.000000 0.00000000383
1168.000000 0.00000000320
1169.000000 0.00000000345
1170.000000 0.00000000498
1171.000000 0.00000000640
1172.000000 0.00000000308
1173.000000 0.00000000510
1174.000000 0.00000000254
1175.000000 0.00000000463
1176.000000 0.00000000444
1177.000000 0.00000000403
1178.000000 0.00000000436
1179.000000 0.00000000469
1180.000000 0.00000000315
1181.000000 0.00000000285
1182.000000 0.00000000209
1183.000000 0.00000000542
1184.000000 0.00000000463
1185.000000 0.00000000246
1186.000000 0.00000000256
1187.000000 0.00000000222
1188.000000 0.00000000243
1189.000000 0.00000000436
1190.000000 0.00000000404
1191.000000 0.00000000197
1192.000000 0.00000000209
1193.000000 0.00000000230
1194.000000 0.00000000208
1195.000000 0.00000000230
1196.000000 0.00000000319
1197.000000 0.00000000289
1198.000000 0.00000000233
1199.000000 0.00000000114
1200.000000 0.00000000184
1201.000000 0.00000000364
1202.000000 0.00000000285
1203.000000 0.00000000097
1204.000000 0.00000000193
1205.000000 0.00000000183
1206.000000 0.00000000264
1207.000000 0.00000000147
1208.000000 0.00000000167
1209.000000 0.00000000132
1210.000000 0.00000000136
1211.000000 0.00000000196
1212.000000 0.00000000115
1213.000000 0.00000000252
1214.000000 0.00000000136
1215.000000 0.00000000134
1216.000000 0.00000000101
1217.000000 0.00000000099
1218.000000 0.00000000221
1219.000000 0.00000000125
1220.000000 0.00000000104
1221.000000 0.00000000084
1222.000000 0.00000000112
1223.000000 0.00000000124
1224.000000 0.00000000116
1225.000000 0.00000000124
1226.000000 0.00000000087
1227.000000 0.00000000093
1228.000000 0.00000000081
1229.000000 0.00000000105
1230.000000 0.00000000099
1231.000000 0.00000000082
1232.000000 0.00000000109
1233.000000 0.00000000114
1234.000000 0.00000000080
1235.000000 0.00000000043
1236.000000 0.00000000088
1237.000000 0.00000000106
1238.000000 0.00000000090
1239.000000 0.00000000034
1240.000000 0.00000000117
1241.000000 0.00000000105
1242.000000 0.00000000037
1243.000000 0.00000000052
1244.000000 0.00000000096
1245.000000 0.00000000071
1246.000000 0.00000000095
1247.000000 0.00000000031
1248.000000 0.00000000070
1249.000000 0.00000000080
1250.000000 0.00000000053
1251.000000 0.00000000056
1252.000000 0.00000000063
1253.000000 0.00000000037
1254.000000 0.00000000060
1255.000000 0.00000000046
1256.000000 0.00000000054
1257.000000 0.00000000053
1258.000000 0.00000000047
1259.000000 0.00000000035
1260.000000 0.00000000074
1261.000000 0.00000000046
1262.000000 0.00000000026
1263.000000 0.00000000048
1264.000000 0.00000000051
1265.000000 0.00000000049
1266.000000 0.00000000051
1267.000000 0.00000000030
1268.000000 0.00000000023
1269.000000 0.00000000035
1270.000000 0.00000000067
1271.000000 0.00000000021
1272.000000 0.00000000033
1273.000000 0.00000000031
1274.000000 0.00000000027
1275.000000 0.00000000037
1276.000000 0.00000000028
1277.000000 0.00000000032
1278.000000 0.00000000017
1279.000000 0.00000000032
1280.000000 0.00000000030
1281.000000 0.00000000032
1282.000000 0.00000000028
1283.000000 0.00000000015
1284.000000 0.00000000022
1285.000000 0.00000000024
1286.000000 0.00000000045
1287.000000 0.00000000023
1288.000000 0.00000000015
1289.000000 0.00000000023
1290.000000 0.00000000019
1291.000000 0.00000000026
1292.000000 0.00000000022
1293.000000 0.00000000024
1294.000000 0.00000000030
1295.000000 0.00000000020
1296.000000 0.00000000022
1297.000000 0.00000000012
1298.000000 0.00000000023
1299.000000 0.00000000033
1300.000000 0.00000000015
1301.000000 0.00000000028
1302.000000 0.00000000012
1303.000000 0.00000000014
1304.000000 0.00000000020
1305.000000 0.00000000025
1306.000000 0.00000000017
1307.000000 0.00000000015
1308.000000 0.00000000015
1309.000000 0.00000000026
1310.000000 0.00000000008


==> data/CG_alone_D100000.tex <==
0.000000 1.00000000000
1.000000 0.51846681054
2.000000 3.13496491545
3.000000 0.67788775851
4.000000 0.49816472596
5.000000 1.03477277932
6.000000 1.64459609122
7.000000 1.17200961761
8.000000 0.68305929970
9.000000 0.50472402959
10.000000 0.58873407240
11.000000 0.73065237870
12.000000 1.07964944962
13.000000 1.03357056117
14.000000 0.87175845950
15.000000 0.57024888290
16.000000 0.54066471664
17.000000 0.48030873103
18.000000 0.53066826504
19.000000 0.69578206750
20.000000 0.89517675177
21.000000 0.90734252448
22.000000 0.60339908680
23.000000 0.51803193826
24.000000 0.47740075595
25.000000 0.49032570813
26.000000 0.49034437221
27.000000 0.55099784738
28.000000 0.61177260463
29.000000 0.68152287484
30.000000 0.69304222477
31.000000 0.65710822478
32.000000 0.53268150277
33.000000 0.44846517401
34.000000 0.42081970683
35.000000 0.43614631032
36.000000 0.46012829348
37.000000 0.56661190571
38.000000 0.60211399862
39.000000 0.60886577741
40.000000 0.58085694595
41.000000 0.54520518349
42.000000 0.43297010335
43.000000 0.43489507000
44.000000 0.41107279701
45.000000 0.41581618847
46.000000 0.43536831277
47.000000 0.50794490097
48.000000 0.55487749945
49.000000 0.62791429241
50.000000 0.50269180699
51.000000 0.40836146205
52.000000 0.42481868883
53.000000 0.37438501954
54.000000 0.39985181623
55.000000 0.44756649299
56.000000 0.43842187891
57.000000 0.42282110611
58.000000 0.54145896793
59.000000 0.54923330207
60.000000 0.44995755304
61.000000 0.39810800346
62.000000 0.38415009919
63.000000 0.37369533573
64.000000 0.36554045508
65.000000 0.38106825975
66.000000 0.44073943594
67.000000 0.43745842289
68.000000 0.45713135964
69.000000 0.47875518282
70.000000 0.41856104376
71.000000 0.39154022619
72.000000 0.33422939255
73.000000 0.34953800573
74.000000 0.38349961355
75.000000 0.38262464150
76.000000 0.35115014296
77.000000 0.39214491268
78.000000 0.43061178472
79.000000 0.39182661084
80.000000 0.41025316989
81.000000 0.34545002675
82.000000 0.38573863925
83.000000 0.32006032903
84.000000 0.32370454960
85.000000 0.30186811323
86.000000 0.33587211690
87.000000 0.37984541946
88.000000 0.38675520601
89.000000 0.36076146551
90.000000 0.34972020691
91.000000 0.37317359071
92.000000 0.30328035721
93.000000 0.31524284205
94.000000 0.29436063698
95.000000 0.25494090062
96.000000 0.30307001211
97.000000 0.39565293918
98.000000 0.36066486834
99.000000 0.31191025824
100.000000 0.26029689265
101.000000 0.29614885148
102.000000 0.32220041604
103.000000 0.32154166438
104.000000 0.27012647454
105.000000 0.23784635781
106.000000 0.27323906097
107.000000 0.27959316906
108.000000 0.29620808975
109.000000 0.30810581892
110.000000 0.27453353037
111.000000 0.26888140211
112.000000 0.25344420318
113.000000 0.23848637427
114.000000 0.18329508297
115.000000 0.21098486806
116.000000 0.26764563480
117.000000 0.22167269916
118.000000 0.26101106028
119.000000 0.22812982300
120.000000 0.18252310943
121.000000 0.17294767285
122.000000 0.17537769537
123.000000 0.15425196184
124.000000 0.16202728339
125.000000 0.16942561315
126.000000 0.12511739243
127.000000 0.29292065079
128.000000 0.10930784287
129.000000 0.12220031797
130.000000 0.13202016399
131.000000 0.25064756771
132.000000 0.10262374591
133.000000 0.23116282960
134.000000 0.10419461019
135.000000 0.26276539999
136.000000 0.10866977975
137.000000 0.26341736776
138.000000 0.10216892618
139.000000 0.24324074963
140.000000 0.09043033534
141.000000 0.14583769494
142.000000 0.19562673249
143.000000 0.09855475098
144.000000 0.20888297129
145.000000 0.11306783213
146.000000 0.09650705250
147.000000 0.23251647414
148.000000 0.08910416174
149.000000 0.10299927580
150.000000 0.24013958814
151.000000 0.10293201605
152.000000 0.07826964316
153.000000 0.17864989994
154.000000 0.15124392301
155.000000 0.06798209562
156.000000 0.11863471577
157.000000 0.19378284335
158.000000 0.08920316296
159.000000 0.06970108672
160.000000 0.17269615379
161.000000 0.16823114940
162.000000 0.06817816649
163.000000 0.06378718968
164.000000 0.12810102772
165.000000 0.17946413397
166.000000 0.07841267435
167.000000 0.05566232521
168.000000 0.12054197042
169.000000 0.15045185301
170.000000 0.06783479339
171.000000 0.05987571570
172.000000 0.10865957375
173.000000 0.15495907108
174.000000 0.07665477655
175.000000 0.05092997645
176.000000 0.06737301419
177.000000 0.12735741262
178.000000 0.12431621406
179.000000 0.05790036901
180.000000 0.05127204949
181.000000 0.07116892557
182.000000 0.13138247309
183.000000 0.10279352542
184.000000 0.05079135400
185.000000 0.04615118694
186.000000 0.06990242604
187.000000 0.13542281445
188.000000 0.08112918941
189.000000 0.04386438234
190.000000 0.04574549405
191.000000 0.06690045798
192.000000 0.10721175048
193.000000 0.08895334635
194.000000 0.05679334175
195.000000 0.04267696879
196.000000 0.04868451587
197.000000 0.08546980578
198.000000 0.09663330285
199.000000 0.06026686450
200.000000 0.04251700243
201.000000 0.04081069203
202.000000 0.06604569082
203.000000 0.08675137800
204.000000 0.08896872757
205.000000 0.04674656697
206.000000 0.03393575705
207.000000 0.04518198694
208.000000 0.06341121925
209.000000 0.09704750152
210.000000 0.06812394199
211.000000 0.03622147850
212.000000 0.03491264589
213.000000 0.04562437014
214.000000 0.07094974959
215.000000 0.07858426587
216.000000 0.06490734437
217.000000 0.03821009551
218.000000 0.03186281468
219.000000 0.04235606898
220.000000 0.06125096586
221.000000 0.07494615949
222.000000 0.05093619948
223.000000 0.03684699684
224.000000 0.03160200512
225.000000 0.03789496775
226.000000 0.06075494178
227.000000 0.06611358176
228.000000 0.06199559278
229.000000 0.03897973743
230.000000 0.02638253227
231.000000 0.03406251633
232.000000 0.05301029818
233.000000 0.05640843583
234.000000 0.06312181316
235.000000 0.03616075030
236.000000 0.02410983029
237.000000 0.03228489107
238.000000 0.05686097889
239.000000 0.05259663860
240.000000 0.03631267555
241.000000 0.02768145353
242.000000 0.02979285599
243.000000 0.05103624509
244.000000 0.04803388260
245.000000 0.04356811431
246.000000 0.03201826605
247.000000 0.02503971773
248.000000 0.03081854580
249.000000 0.08466953418
250.000000 0.03353320724
251.000000 0.02196257976
252.000000 0.02918978660
253.000000 0.07508951032
254.000000 0.04505660203
255.000000 0.03480855812
256.000000 0.02700000290
257.000000 0.02478170760
258.000000 0.05055876977
259.000000 0.03955676795
260.000000 0.06957634785
261.000000 0.02918354678
262.000000 0.04090658089
263.000000 0.02093888069
264.000000 0.05750294402
265.000000 0.04360097510
266.000000 0.06013151876
267.000000 0.03080358848
268.000000 0.03967871850
269.000000 0.02074754072
270.000000 0.05530751580
271.000000 0.03647213023
272.000000 0.06612355123
273.000000 0.04102644834
274.000000 0.02923629927
275.000000 0.03715108182
276.000000 0.02346603957
277.000000 0.07107404090
278.000000 0.04303931143
279.000000 0.06705545778
280.000000 0.03846224180
281.000000 0.02481485870
282.000000 0.04601898748
283.000000 0.04002767575
284.000000 0.07802126110
285.000000 0.07777255580
286.000000 0.02874436800
287.000000 0.05796020440
288.000000 0.04472360440
289.000000 0.04718731784
290.000000 0.09739353240
291.000000 0.05618073083
292.000000 0.05590272347
293.000000 0.08047484908
294.000000 0.03548821105
295.000000 0.03333062555
296.000000 0.07037418558
297.000000 0.05765327745
298.000000 0.04327295777
299.000000 0.06802767667
300.000000 0.03230538679
301.000000 0.01858820925
302.000000 0.02993583581
303.000000 0.02028391729
304.000000 0.01967226090
305.000000 0.03506145543
306.000000 0.02080682662
307.000000 0.00784044483
308.000000 0.00784763507
309.000000 0.01112038231
310.000000 0.00676154620
311.000000 0.00530376334
312.000000 0.01035987669
313.000000 0.00596325226
314.000000 0.00234632569
315.000000 0.00244586879
316.000000 0.00337113679
317.000000 0.00227387784
318.000000 0.00182081007
319.000000 0.00315026084
320.000000 0.00268971753
321.000000 0.00126638359
322.000000 0.00146771245
323.000000 0.00189144623
324.000000 0.00131511861
325.000000 0.00136549488
326.000000 0.00229432563
327.000000 0.00260272761
328.000000 0.00125293952
329.000000 0.00138049574
330.000000 0.00178144221
331.000000 0.00124871936
332.000000 0.00077088239
333.000000 0.00126050083
334.000000 0.00178264753
335.000000 0.00119703000
336.000000 0.00047673973
337.000000 0.00067378737
338.000000 0.00088289626
339.000000 0.00072053105
340.000000 0.00056959974
341.000000 0.00093641265
342.000000 0.00114457193
343.000000 0.00074364373
344.000000 0.00042814133
345.000000 0.00060694567
346.000000 0.00078970383
347.000000 0.00048316953
348.000000 0.00063166646
349.000000 0.00086913891
350.000000 0.00057378501
351.000000 0.00028527664
352.000000 0.00033901662
353.000000 0.00046595190
354.000000 0.00045553496
355.000000 0.00034967800
356.000000 0.00052973311
357.000000 0.00065185566
358.000000 0.00039036013
359.000000 0.00023925509
360.000000 0.00031405022
361.000000 0.00052793667
362.000000 0.00034412055
363.000000 0.00021467209
364.000000 0.00030546774
365.000000 0.00030800020
366.000000 0.00023417636
367.000000 0.00020727626
368.000000 0.00040320272
369.000000 0.00032291354
370.000000 0.00030270976
371.000000 0.00016390692
372.000000 0.00027045175
373.000000 0.00052956560
374.000000 0.00029278104
375.000000 0.00014197162
376.000000 0.00018472245
377.000000 0.00032185417
378.000000 0.00024432012
379.000000 0.00018923900
380.000000 0.00023628200
381.000000 0.00031836689
382.000000 0.00025455795
383.000000 0.00012481506
384.000000 0.00029906679
385.000000 0.00026367299
386.000000 0.00039236818
387.000000 0.00014219374
388.000000 0.00012149239
389.000000 0.00017602651
390.000000 0.00024425068
391.000000 0.00027129071
392.000000 0.00013752548
393.000000 0.00029214097
394.000000 0.00021592800
395.000000 0.00024795608
396.000000 0.00009121824
397.000000 0.00021024590
398.000000 0.00021761486
399.000000 0.00034387756
400.000000 0.00011583521
401.000000 0.00012260042
402.000000 0.00012918078
403.000000 0.00014864458
404.000000 0.00028900759
405.000000 0.00018650248
406.000000 0.00020192122
407.000000 0.00008870687
408.000000 0.00023026072
409.000000 0.00013749522
410.000000 0.00012799878
411.000000 0.00011906270
412.000000 0.00014349914
413.000000 0.00021208758
414.000000 0.00016924869
415.000000 0.00017690236
416.000000 0.00008972964
417.000000 0.00011495845
418.000000 0.00013844636
419.000000 0.00015641573
420.000000 0.00025136289
421.000000 0.00008355093
422.000000 0.00009544634
423.000000 0.00010139942
424.000000 0.00010806963
425.000000 0.00024009622
426.000000 0.00011730486
427.000000 0.00008940474
428.000000 0.00012170573
429.000000 0.00009921375
430.000000 0.00016023583
431.000000 0.00013354791
432.000000 0.00007169493
433.000000 0.00011065578
434.000000 0.00009864654
435.000000 0.00009401725
436.000000 0.00016173003
437.000000 0.00008886212
438.000000 0.00006686257
439.000000 0.00009509324
440.000000 0.00006998574
441.000000 0.00010278990
442.000000 0.00015314074
443.000000 0.00006180928
444.000000 0.00005595666
445.000000 0.00006095419
446.000000 0.00006346179
447.000000 0.00013135630
448.000000 0.00008400557
449.000000 0.00004782486
450.000000 0.00007153656
451.000000 0.00007033054
452.000000 0.00006353384
453.000000 0.00008447475
454.000000 0.00005305948
455.000000 0.00003868275
456.000000 0.00007761947
457.000000 0.00005542092
458.000000 0.00006297716
459.000000 0.00007358351
460.000000 0.00003550393
461.000000 0.00003213309
462.000000 0.00005699862
463.000000 0.00005742574
464.000000 0.00006278783
465.000000 0.00006816115
466.000000 0.00003660889
467.000000 0.00002090521
468.000000 0.00003704442
469.000000 0.00006852839
470.000000 0.00003410586
471.000000 0.00003407892
472.000000 0.00002927480
473.000000 0.00002095374
474.000000 0.00003937888
475.000000 0.00004851443
476.000000 0.00001713542
477.000000 0.00002718741
478.000000 0.00003052477
479.000000 0.00002349228
480.000000 0.00003327052
481.000000 0.00004294242
482.000000 0.00002198597
483.000000 0.00002209632
484.000000 0.00002171297
485.000000 0.00002259915
486.000000 0.00002137031
487.000000 0.00003977775
488.000000 0.00001837312
489.000000 0.00001440407
490.000000 0.00002065438
491.000000 0.00003252834
492.000000 0.00002408118
493.000000 0.00001862929
494.000000 0.00002515674
495.000000 0.00001477364
496.000000 0.00002035824
497.000000 0.00003304329
498.000000 0.00001936258
499.000000 0.00001266046
500.000000 0.00002726826
501.000000 0.00003158632
502.000000 0.00002363924
503.000000 0.00001261953
504.000000 0.00001167609
505.000000 0.00003170877
506.000000 0.00002833465
507.000000 0.00001504179
508.000000 0.00001508266
509.000000 0.00001652809
510.000000 0.00002152906
511.000000 0.00001740205
512.000000 0.00002259422
513.000000 0.00003113354
514.000000 0.00001605877
515.000000 0.00001626830
516.000000 0.00001095625
517.000000 0.00003166292
518.000000 0.00002297668
519.000000 0.00001658955
520.000000 0.00002298684
521.000000 0.00001381743
522.000000 0.00001717703
523.000000 0.00001730521
524.000000 0.00002961225
525.000000 0.00001566086
526.000000 0.00001580818
527.000000 0.00001299926
528.000000 0.00003006024
529.000000 0.00001524192
530.000000 0.00002020595
531.000000 0.00002208189
532.000000 0.00002048308
533.000000 0.00001202122
534.000000 0.00001067644
535.000000 0.00003405599
536.000000 0.00001623621
537.000000 0.00001896363
538.000000 0.00001195813
539.000000 0.00001697605
540.000000 0.00001428130
541.000000 0.00001299050
542.000000 0.00001627002
543.000000 0.00002964468
544.000000 0.00001321810
545.000000 0.00000981144
546.000000 0.00001094129
547.000000 0.00001714161
548.000000 0.00003038664
549.000000 0.00001574670
550.000000 0.00001575987
551.000000 0.00000953179
552.000000 0.00001552706
553.000000 0.00001524372
554.000000 0.00001250942
555.000000 0.00002304317
556.000000 0.00001705856
557.000000 0.00002167251
558.000000 0.00001048150
559.000000 0.00000894356
560.000000 0.00002284310
561.000000 0.00002631665
562.000000 0.00001468923
563.000000 0.00001274448
564.000000 0.00001146985
565.000000 0.00001907677
566.000000 0.00002236005
567.000000 0.00001443851
568.000000 0.00001855427
569.000000 0.00002327594
570.000000 0.00002248938
571.000000 0.00001950857
572.000000 0.00001001521
573.000000 0.00001491299
574.000000 0.00002550488
575.000000 0.00002040841
576.000000 0.00002382450
577.000000 0.00001105802
578.000000 0.00001704489
579.000000 0.00002570400
580.000000 0.00001741875
581.000000 0.00002006200
582.000000 0.00001265874
583.000000 0.00002108679
584.000000 0.00001851343
585.000000 0.00001368373
586.000000 0.00002260084
587.000000 0.00001738653
588.000000 0.00002601783
589.000000 0.00001289121
590.000000 0.00001053461
591.000000 0.00002243428
592.000000 0.00003302657
593.000000 0.00001598090
594.000000 0.00001551623
595.000000 0.00001199084
596.000000 0.00001598828
597.000000 0.00001308952
598.000000 0.00001271894
599.000000 0.00002472787
600.000000 0.00002494445
601.000000 0.00001680273
602.000000 0.00001465870
603.000000 0.00000754366
604.000000 0.00001567586
605.000000 0.00002829519
606.000000 0.00001418077
607.000000 0.00001051595
608.000000 0.00001340656
609.000000 0.00001259199
610.000000 0.00001612651
611.000000 0.00001738769
612.000000 0.00001270054
613.000000 0.00001449483
614.000000 0.00002561656
615.000000 0.00001219599
616.000000 0.00000990728
617.000000 0.00001203758
618.000000 0.00001018067
619.000000 0.00002427079
620.000000 0.00001114909
621.000000 0.00001164451
622.000000 0.00001079312
623.000000 0.00000843736
624.000000 0.00001664981
625.000000 0.00001957551
626.000000 0.00001522382
627.000000 0.00000897988
628.000000 0.00001171521
629.000000 0.00001108721
630.000000 0.00001313581
631.000000 0.00002966207
632.000000 0.00001663199
633.000000 0.00000872843
634.000000 0.00001226393
635.000000 0.00001374901
636.000000 0.00001590320
637.000000 0.00001342788
638.000000 0.00001488575
639.000000 0.00001781255
640.000000 0.00001741795
641.000000 0.00001582364
642.000000 0.00000940738
643.000000 0.00001035741
644.000000 0.00002813084
645.000000 0.00001804821
646.000000 0.00001351497
647.000000 0.00001353837
648.000000 0.00001158073
649.000000 0.00001185920
650.000000 0.00001973915
651.000000 0.00002658558
652.000000 0.00001513892
653.000000 0.00000961061
654.000000 0.00001292269
655.000000 0.00001611430
656.000000 0.00001416658
657.000000 0.00001578482
658.000000 0.00001979909
659.000000 0.00001148106
660.000000 0.00001061816
661.000000 0.00001534193
662.000000 0.00001768146
663.000000 0.00001034266
664.000000 0.00001274396
665.000000 0.00001325841
666.000000 0.00002109255
667.000000 0.00001175976
668.000000 0.00001621550
669.000000 0.00000899562
670.000000 0.00001136389
671.000000 0.00001107624
672.000000 0.00002232904
673.000000 0.00001293009
674.000000 0.00000837568
675.000000 0.00000684756
676.000000 0.00002305106
677.000000 0.00001185723
678.000000 0.00000870249
679.000000 0.00000677851
680.000000 0.00000905122
681.000000 0.00002028872
682.000000 0.00001122836
683.000000 0.00001161294
684.000000 0.00000849310
685.000000 0.00001103774
686.000000 0.00000630711
687.000000 0.00000727619
688.000000 0.00001909389
689.000000 0.00000860761
690.000000 0.00000687830
691.000000 0.00000699035
692.000000 0.00001268377
693.000000 0.00000734371
694.000000 0.00000776085
695.000000 0.00001331464
696.000000 0.00000643222
697.000000 0.00000997655
698.000000 0.00000963262
699.000000 0.00000921773
700.000000 0.00000656619
701.000000 0.00000483763
702.000000 0.00000893487
703.000000 0.00001240111
704.000000 0.00001167253
705.000000 0.00000720342
706.000000 0.00000368290
707.000000 0.00000742569
708.000000 0.00001256190
709.000000 0.00000889307
710.000000 0.00000389041
711.000000 0.00000436670
712.000000 0.00001516244
713.000000 0.00000759838
714.000000 0.00000484377
715.000000 0.00000612261
716.000000 0.00000561761
717.000000 0.00000873361
718.000000 0.00000759364
719.000000 0.00000812484
720.000000 0.00000811139
721.000000 0.00000636506
722.000000 0.00000715111
723.000000 0.00000425466
724.000000 0.00000974277
725.000000 0.00000731943
726.000000 0.00000507131
727.000000 0.00000765992
728.000000 0.00000680001
729.000000 0.00000936294
730.000000 0.00000577288
731.000000 0.00000605965
732.000000 0.00000629981
733.000000 0.00000419167
734.000000 0.00000934233
735.000000 0.00001187977
736.000000 0.00000530228
737.000000 0.00000468786
738.000000 0.00000419417
739.000000 0.00000707473
740.000000 0.00000932917
741.000000 0.00000736873
742.000000 0.00000578350
743.000000 0.00000746851
744.000000 0.00000464563
745.000000 0.00000393349
746.000000 0.00000597115
747.000000 0.00000835858
748.000000 0.00000946161
749.000000 0.00000594836
750.000000 0.00000303163
751.000000 0.00000574908
752.000000 0.00000960022
753.000000 0.00000534221
754.000000 0.00000438944
755.000000 0.00000773775
756.000000 0.00000399981
757.000000 0.00000588027
758.000000 0.00000380766
759.000000 0.00000553393
760.000000 0.00000494431
761.000000 0.00000321490
762.000000 0.00000593893
763.000000 0.00000767511
764.000000 0.00000481002
765.000000 0.00000478162
766.000000 0.00000227397
767.000000 0.00000612798
768.000000 0.00000737073
769.000000 0.00000401913
770.000000 0.00000508648
771.000000 0.00000361665
772.000000 0.00000388682
773.000000 0.00000311914
774.000000 0.00000385021
775.000000 0.00000312960
776.000000 0.00000680990
777.000000 0.00000588550
778.000000 0.00000330237
779.000000 0.00000210357
780.000000 0.00000307559
781.000000 0.00000356625
782.000000 0.00000518121
783.000000 0.00000559362
784.000000 0.00000310001
785.000000 0.00000232451
786.000000 0.00000207763
787.000000 0.00000367564
788.000000 0.00000343862
789.000000 0.00000555005
790.000000 0.00000384840
791.000000 0.00000282137
792.000000 0.00000150762
793.000000 0.00000353937
794.000000 0.00000458480
795.000000 0.00000337223
796.000000 0.00000169161
797.000000 0.00000323432
798.000000 0.00000244537
799.000000 0.00000237299
800.000000 0.00000296316
801.000000 0.00000317479
802.000000 0.00000235140
803.000000 0.00000379876
804.000000 0.00000198652
805.000000 0.00000182154
806.000000 0.00000197341
807.000000 0.00000414345
808.000000 0.00000209019
809.000000 0.00000239990
810.000000 0.00000186513
811.000000 0.00000163302
812.000000 0.00000201603
813.000000 0.00000435437
814.000000 0.00000248688
815.000000 0.00000214009
816.000000 0.00000178206
817.000000 0.00000146211
818.000000 0.00000216991
819.000000 0.00000287685
820.000000 0.00000203830
821.000000 0.00000186448
822.000000 0.00000196071
823.000000 0.00000237978
824.000000 0.00000202079
825.000000 0.00000130719
826.000000 0.00000317552
827.000000 0.00000253644
828.000000 0.00000185540
829.000000 0.00000143340
830.000000 0.00000160712
831.000000 0.00000285161
832.000000 0.00000167532
833.000000 0.00000190225
834.000000 0.00000274262
835.000000 0.00000177656
836.000000 0.00000202726
837.000000 0.00000219789
838.000000 0.00000157915
839.000000 0.00000126520
840.000000 0.00000263717
841.000000 0.00000265733
842.000000 0.00000145183
843.000000 0.00000115688
844.000000 0.00000226170
845.000000 0.00000285436
846.000000 0.00000098349
847.000000 0.00000145699
848.000000 0.00000155687
849.000000 0.00000144910
850.000000 0.00000240473
851.000000 0.00000160426
852.000000 0.00000113557
853.000000 0.00000114745
854.000000 0.00000111095
855.000000 0.00000227315
856.000000 0.00000149831
857.000000 0.00000237575
858.000000 0.00000096001
859.000000 0.00000109820
860.000000 0.00000122039
861.000000 0.00000180482
862.000000 0.00000272403
863.000000 0.00000129448
864.000000 0.00000121245
865.000000 0.00000224157
866.000000 0.00000125490
867.000000 0.00000106132
868.000000 0.00000126027
869.000000 0.00000120249
870.000000 0.00000304407
871.000000 0.00000216309
872.000000 0.00000058730
873.000000 0.00000137168
874.000000 0.00000207899
875.000000 0.00000162345
876.000000 0.00000066991
877.000000 0.00000073444
878.000000 0.00000198663
879.000000 0.00000173864
880.000000 0.00000130329
881.000000 0.00000086104
882.000000 0.00000066866
883.000000 0.00000094845
884.000000 0.00000121257
885.000000 0.00000088392
886.000000 0.00000148166
887.000000 0.00000123593
888.000000 0.00000044883
889.000000 0.00000139386
890.000000 0.00000131749
891.000000 0.00000078086
892.000000 0.00000071661
893.000000 0.00000118469
894.000000 0.00000107549
895.000000 0.00000073480
896.000000 0.00000085086
897.000000 0.00000090173
898.000000 0.00000074483
899.000000 0.00000075018
900.000000 0.00000086530
901.000000 0.00000125558
902.000000 0.00000068001
903.000000 0.00000094661
904.000000 0.00000058480
905.000000 0.00000137479
906.000000 0.00000060505
907.000000 0.00000049596
908.000000 0.00000067428
909.000000 0.00000114790
910.000000 0.00000107506
911.000000 0.00000123248
912.000000 0.00000042891
913.000000 0.00000048169
914.000000 0.00000112071
915.000000 0.00000139591
916.000000 0.00000050547
917.000000 0.00000057324
918.000000 0.00000074011
919.000000 0.00000085024
920.000000 0.00000058872
921.000000 0.00000131450
922.000000 0.00000065270
923.000000 0.00000068156
924.000000 0.00000069379
925.000000 0.00000071278
926.000000 0.00000070209
927.000000 0.00000051010
928.000000 0.00000059529
929.000000 0.00000077951
930.000000 0.00000103875
931.000000 0.00000049993
932.000000 0.00000060967
933.000000 0.00000055869
934.000000 0.00000080574
935.000000 0.00000096254
936.000000 0.00000140044
937.000000 0.00000049465
938.000000 0.00000050108
939.000000 0.00000078258
940.000000 0.00000058701
941.000000 0.00000065260
942.000000 0.00000104634
943.000000 0.00000085314
944.000000 0.00000060336
945.000000 0.00000063074
946.000000 0.00000041299
947.000000 0.00000051332
948.000000 0.00000141004
949.000000 0.00000077536
950.000000 0.00000050844
951.000000 0.00000042124
952.000000 0.00000065474
953.000000 0.00000059571
954.000000 0.00000079818
955.000000 0.00000092986
956.000000 0.00000063074
957.000000 0.00000074153
958.000000 0.00000063539
959.000000 0.00000045552
960.000000 0.00000036867
961.000000 0.00000086630
962.000000 0.00000072291
963.000000 0.00000072504
964.000000 0.00000075055
965.000000 0.00000033770
966.000000 0.00000037237
967.000000 0.00000075874
968.000000 0.00000088946
969.000000 0.00000078078
970.000000 0.00000032239
971.000000 0.00000044909
972.000000 0.00000052293
973.000000 0.00000055856
974.000000 0.00000042788
975.000000 0.00000076815
976.000000 0.00000045434
977.000000 0.00000038095
978.000000 0.00000035086
979.000000 0.00000059334
980.000000 0.00000040084
981.000000 0.00000072005
982.000000 0.00000041805
983.000000 0.00000023854
984.000000 0.00000047516
985.000000 0.00000062795
986.000000 0.00000040547
987.000000 0.00000040983
988.000000 0.00000037695
989.000000 0.00000036811
990.000000 0.00000025562
991.000000 0.00000058009
992.000000 0.00000025708
993.000000 0.00000046863
994.000000 0.00000051173
995.000000 0.00000019282
996.000000 0.00000029766
997.000000 0.00000035995
998.000000 0.00000037956
999.000000 0.00000026591
1000.000000 0.00000033224
1001.000000 0.00000029668
1002.000000 0.00000016739
1003.000000 0.00000031531
1004.000000 0.00000034619
1005.000000 0.00000030757
1006.000000 0.00000022568
1007.000000 0.00000016093
1008.000000 0.00000035857
1009.000000 0.00000013364
1010.000000 0.00000023800
1011.000000 0.00000034969
1012.000000 0.00000023713
1013.000000 0.00000035262
1014.000000 0.00000018389
1015.000000 0.00000015379
1016.000000 0.00000021189
1017.000000 0.00000018040
1018.000000 0.00000042875
1019.000000 0.00000020196
1020.000000 0.00000011369
1021.000000 0.00000024014
1022.000000 0.00000022757
1023.000000 0.00000018764
1024.000000 0.00000018324
1025.000000 0.00000012754
1026.000000 0.00000023494
1027.000000 0.00000019612
1028.000000 0.00000011419
1029.000000 0.00000014408
1030.000000 0.00000023318
1031.000000 0.00000017695
1032.000000 0.00000018982
1033.000000 0.00000015629
1034.000000 0.00000025213
1035.000000 0.00000021486
1036.000000 0.00000013804
1037.000000 0.00000013402
1038.000000 0.00000013969
1039.000000 0.00000012461
1040.000000 0.00000020509
1041.000000 0.00000032305
1042.000000 0.00000010133
1043.000000 0.00000012026
1044.000000 0.00000013080
1045.000000 0.00000019222
1046.000000 0.00000020558
1047.000000 0.00000018110
1048.000000 0.00000023859
1049.000000 0.00000007279
1050.000000 0.00000014377
1051.000000 0.00000029371
1052.000000 0.00000013924
1053.000000 0.00000010447
1054.000000 0.00000016177
1055.000000 0.00000017462
1056.000000 0.00000009385
1057.000000 0.00000018848
1058.000000 0.00000024372
1059.000000 0.00000014695
1060.000000 0.00000015937
1061.000000 0.00000007190
1062.000000 0.00000015250
1063.000000 0.00000019404
1064.000000 0.00000017006
1065.000000 0.00000010749
1066.000000 0.00000010905
1067.000000 0.00000010676
1068.000000 0.00000023100
1069.000000 0.00000016486
1070.000000 0.00000007248
1071.000000 0.00000015349
1072.000000 0.00000020212
1073.000000 0.00000006838
1074.000000 0.00000009144
1075.000000 0.00000016765
1076.000000 0.00000011341
1077.000000 0.00000008580
1078.000000 0.00000013433
1079.000000 0.00000016066
1080.000000 0.00000011947
1081.000000 0.00000010111
1082.000000 0.00000006238
1083.000000 0.00000008498
1084.000000 0.00000012520
1085.000000 0.00000014168
1086.000000 0.00000009826
1087.000000 0.00000011025
1088.000000 0.00000008428
1089.000000 0.00000006472
1090.000000 0.00000006017
1091.000000 0.00000009769
1092.000000 0.00000017971
1093.000000 0.00000005099
1094.000000 0.00000006381
1095.000000 0.00000009347
1096.000000 0.00000009210
1097.000000 0.00000011486
1098.000000 0.00000012881
1099.000000 0.00000009652
1100.000000 0.00000007779
1101.000000 0.00000007169
1102.000000 0.00000005182
1103.000000 0.00000007116
1104.000000 0.00000009544
1105.000000 0.00000015634
1106.000000 0.00000010557
1107.000000 0.00000004503
1108.000000 0.00000005309
1109.000000 0.00000007571
1110.000000 0.00000015255
1111.000000 0.00000006097
1112.000000 0.00000005420
1113.000000 0.00000004150
1114.000000 0.00000010051
1115.000000 0.00000008789
1116.000000 0.00000008696
1117.000000 0.00000005639
1118.000000 0.00000006533
1119.000000 0.00000004653
1120.000000 0.00000005520
1121.000000 0.00000005554
1122.000000 0.00000006940
1123.000000 0.00000006539
1124.000000 0.00000006194
1125.000000 0.00000006075
1126.000000 0.00000003824
1127.000000 0.00000009386
1128.000000 0.00000003192
1129.000000 0.00000007420
1130.000000 0.00000004785
1131.000000 0.00000006942
1132.000000 0.00000005961
1133.000000 0.00000003178
1134.000000 0.00000004174
1135.000000 0.00000004894
1136.000000 0.00000006421
1137.000000 0.00000005749
1138.000000 0.00000004224
1139.000000 0.00000002872
1140.000000 0.00000003026
1141.000000 0.00000004498
1142.000000 0.00000005921
1143.000000 0.00000002133
1144.000000 0.00000002470
1145.000000 0.00000004770
1146.000000 0.00000005321
1147.000000 0.00000005641
1148.000000 0.00000002189
1149.000000 0.00000002560
1150.000000 0.00000003183
1151.000000 0.00000002883
1152.000000 0.00000003746
1153.000000 0.00000003173
1154.000000 0.00000003239
1155.000000 0.00000003395
1156.000000 0.00000002965
1157.000000 0.00000002944
1158.000000 0.00000002047
1159.000000 0.00000002626
1160.000000 0.00000002519
1161.000000 0.00000001928
1162.000000 0.00000003040
1163.000000 0.00000003649
1164.000000 0.00000001889
1165.000000 0.00000002671
1166.000000 0.00000001194
1167.000000 0.00000002904
1168.000000 0.00000003132
1169.000000 0.00000001721
1170.000000 0.00000001901
1171.000000 0.00000001939
1172.000000 0.00000002618
1173.000000 0.00000002329
1174.000000 0.00000001873
1175.000000 0.00000001746
1176.000000 0.00000002724
1177.000000 0.00000001402
1178.000000 0.00000001781
1179.000000 0.00000003207
1180.000000 0.00000001867
1181.000000 0.00000002000
1182.000000 0.00000001263
1183.000000 0.00000002123
1184.000000 0.00000001403
1185.000000 0.00000003144
1186.000000 0.00000002514
1187.000000 0.00000001589
1188.000000 0.00000001000
1189.000000 0.00000001370
1190.000000 0.00000004070
1191.000000 0.00000002422
1192.000000 0.00000001112
1193.000000 0.00000001442
1194.000000 0.00000001273
1195.000000 0.00000001994
1196.000000 0.00000003015
1197.000000 0.00000001897
1198.000000 0.00000001527
1199.000000 0.00000002090
1200.000000 0.00000001062
1201.000000 0.00000001251
1202.000000 0.00000002293
1203.000000 0.00000003519
1204.000000 0.00000001570
1205.000000 0.00000001683
1206.000000 0.00000001077
1207.000000 0.00000001876
1208.000000 0.00000002135
1209.000000 0.00000001581
1210.000000 0.00000001660
1211.000000 0.00000002902
1212.000000 0.00000001363
1213.000000 0.00000001046
1214.000000 0.00000002360
1215.000000 0.00000001735
1216.000000 0.00000001229
1217.000000 0.00000001648
1218.000000 0.00000002093
1219.000000 0.00000001399
1220.000000 0.00000002115
1221.000000 0.00000001124
1222.000000 0.00000000970
1223.000000 0.00000001600
1224.000000 0.00000001684
1225.000000 0.00000002417
1226.000000 0.00000001555
1227.000000 0.00000000927
1228.000000 0.00000000995
1229.000000 0.00000001172
1230.000000 0.00000002129
1231.000000 0.00000002034
1232.000000 0.00000001145
1233.000000 0.00000000780
1234.000000 0.00000000959
1235.000000 0.00000001145
1236.000000 0.00000001611
1237.000000 0.00000001143
1238.000000 0.00000001464
1239.000000 0.00000001163
1240.000000 0.00000000592
1241.000000 0.00000000724
1242.000000 0.00000002017
1243.000000 0.00000000810
1244.000000 0.00000000605
1245.000000 0.00000000652
1246.000000 0.00000001342
1247.000000 0.00000001281
1248.000000 0.00000000992
1249.000000 0.00000000588
1250.000000 0.00000000905
1251.000000 0.00000001020
1252.000000 0.00000000610
1253.000000 0.00000000665
1254.000000 0.00000000836
1255.000000 0.00000001452
1256.000000 0.00000000671
1257.000000 0.00000000445
1258.000000 0.00000000521
1259.000000 0.00000000980
1260.000000 0.00000000467
1261.000000 0.00000000419
1262.000000 0.00000000515
1263.000000 0.00000001182
1264.000000 0.00000000658
1265.000000 0.00000000391
1266.000000 0.00000000622
1267.000000 0.00000000505
1268.000000 0.00000000618
1269.000000 0.00000000569
1270.000000 0.00000000494
1271.000000 0.00000000566
1272.000000 0.00000000586
1273.000000 0.00000000583
1274.000000 0.00000000441
1275.000000 0.00000000332
1276.000000 0.00000000618
1277.000000 0.00000000499
1278.000000 0.00000000424
1279.000000 0.00000000354
1280.000000 0.00000000396
1281.000000 0.00000000414
1282.000000 0.00000000547
1283.000000 0.00000000476
1284.000000 0.00000000245
1285.000000 0.00000000398
1286.000000 0.00000000368
1287.000000 0.00000000289
1288.000000 0.00000000698
1289.000000 0.00000000391
1290.000000 0.00000000312
1291.000000 0.00000000309
1292.000000 0.00000000240
1293.000000 0.00000000345
1294.000000 0.00000000462
1295.000000 0.00000000390
1296.000000 0.00000000235
1297.000000 0.00000000278
1298.000000 0.00000000447
1299.000000 0.00000000386
1300.000000 0.00000000160
1301.000000 0.00000000246
1302.000000 0.00000000224
1303.000000 0.00000000386
1304.000000 0.00000000319
1305.000000 0.00000000268
1306.000000 0.00000000342
1307.000000 0.00000000148
1308.000000 0.00000000190
1309.000000 0.00000000209
1310.000000 0.00000000277
1311.000000 0.00000000412
1312.000000 0.00000000223
1313.000000 0.00000000236
1314.000000 0.00000000124
1315.000000 0.00000000228
1316.000000 0.00000000245
1317.000000 0.00000000195
1318.000000 0.00000000143
1319.000000 0.00000000357
1320.000000 0.00000000159
1321.000000 0.00000000109
1322.000000 0.00000000197
1323.000000 0.00000000145
1324.000000 0.00000000224
1325.000000 0.00000000193
1326.000000 0.00000000206
1327.000000 0.00000000169
1328.000000 0.00000000149
1329.000000 0.00000000186
1330.000000 0.00000000119
1331.000000 0.00000000219
1332.000000 0.00000000116
1333.000000 0.00000000127
1334.000000 0.00000000195
1335.000000 0.00000000204
1336.000000 0.00000000198
1337.000000 0.00000000076
1338.000000 0.00000000080
1339.000000 0.00000000242
1340.000000 0.00000000168
1341.000000 0.00000000142
1342.000000 0.00000000093
1343.000000 0.00000000059
1344.000000 0.00000000113
1345.000000 0.00000000107
1346.000000 0.00000000149
1347.000000 0.00000000153
1348.000000 0.00000000066
1349.000000 0.00000000048
1350.000000 0.00000000105
1351.000000 0.00000000203
1352.000000 0.00000000071
1353.000000 0.00000000049
1354.000000 0.00000000061
1355.000000 0.00000000134
1356.000000 0.00000000102
1357.000000 0.00000000084
1358.000000 0.00000000091
1359.000000 0.00000000060
1360.000000 0.00000000042
1361.000000 0.00000000113
1362.000000 0.00000000067
1363.000000 0.00000000083
1364.000000 0.00000000064
1365.000000 0.00000000051
1366.000000 0.00000000058
1367.000000 0.00000000052
1368.000000 0.00000000062
1369.000000 0.00000000093
1370.000000 0.00000000040
1371.000000 0.00000000040
1372.000000 0.00000000068
1373.000000 0.00000000041
1374.000000 0.00000000108
1375.000000 0.00000000053
1376.000000 0.00000000029
1377.000000 0.00000000032
1378.000000 0.00000000062
1379.000000 0.00000000051
1380.000000 0.00000000040
1381.000000 0.00000000042
1382.000000 0.00000000042
1383.000000 0.00000000043
1384.000000 0.00000000022
1385.000000 0.00000000065
1386.000000 0.00000000031
1387.000000 0.00000000037
1388.000000 0.00000000036
1389.000000 0.00000000040
1390.000000 0.00000000031
1391.000000 0.00000000033
1392.000000 0.00000000018
1393.000000 0.00000000027
1394.000000 0.00000000043
1395.000000 0.00000000029
1396.000000 0.00000000016
1397.000000 0.00000000030
1398.000000 0.00000000036
1399.000000 0.00000000030
1400.000000 0.00000000020
1401.000000 0.00000000016
1402.000000 0.00000000031
1403.000000 0.00000000028
1404.000000 0.00000000026
1405.000000 0.00000000025
1406.000000 0.00000000026
1407.000000 0.00000000016
1408.000000 0.00000000016
1409.000000 0.00000000024
1410.000000 0.00000000027
1411.000000 0.00000000016
1412.000000 0.00000000027
1413.000000 0.00000000020
1414.000000 0.00000000020
1415.000000 0.00000000019
1416.000000 0.00000000019
1417.000000 0.00000000031
1418.000000 0.00000000024
1419.000000 0.00000000016
1420.000000 0.00000000014
1421.000000 0.00000000016
1422.000000 0.00000000036
1423.000000 0.00000000010


==> data/CG_alone_D1000000.tex <==
0.000000 1.00000000000
1.000000 0.51832027216
2.000000 3.14079650641
3.000000 0.67956415183
4.000000 0.49742505984
5.000000 1.03080240293
6.000000 1.64454331827
7.000000 1.17681700893
8.000000 0.68605820960
9.000000 0.50568852867
10.000000 0.58806115476
11.000000 0.72867268108
12.000000 1.07772827192
13.000000 1.03409830872
14.000000 0.87412042774
15.000000 0.57216952540
16.000000 0.54222037920
17.000000 0.48113603151
18.000000 0.53086956817
19.000000 0.69545249533
20.000000 0.89471569877
21.000000 0.90738292900
22.000000 0.60384310366
23.000000 0.51869170386
24.000000 0.47825817064
25.000000 0.49137480797
26.000000 0.49140977985
27.000000 0.55199531289
28.000000 0.61251206025
29.000000 0.68184795844
30.000000 0.69287490666
31.000000 0.65675656206
32.000000 0.53253188191
33.000000 0.44873795387
34.000000 0.42156786471
35.000000 0.43735029269
36.000000 0.46156996903
37.000000 0.56811468013
38.000000 0.60297020790
39.000000 0.60880855491
40.000000 0.58014233728
41.000000 0.54437721249
42.000000 0.43269383979
43.000000 0.43532001250
44.000000 0.41217665925
45.000000 0.41750447083
46.000000 0.43730999019
47.000000 0.50972152090
48.000000 0.55552360864
49.000000 0.62711028399
50.000000 0.50085921297
51.000000 0.40719564688
52.000000 0.42454336047
53.000000 0.37521086501
54.000000 0.40183941026
55.000000 0.45023151187
56.000000 0.44080827731
57.000000 0.42435257393
58.000000 0.54184718152
59.000000 0.54731947849
60.000000 0.44750226078
61.000000 0.39634339532
62.000000 0.38364732167
63.000000 0.37471636502
64.000000 0.36790613058
65.000000 0.38437697784
66.000000 0.44427455761
67.000000 0.43943769685
68.000000 0.45716719157
69.000000 0.47667910991
70.000000 0.41566307585
71.000000 0.38901235629
72.000000 0.33332487434
73.000000 0.35044330187
74.000000 0.38609485217
75.000000 0.38607004063
76.000000 0.35438548235
77.000000 0.39495920161
78.000000 0.43152595613
79.000000 0.39056975988
80.000000 0.40730744847
81.000000 0.34272008567
82.000000 0.38339773565
83.000000 0.31951048480
84.000000 0.32510313946
85.000000 0.30477225148
86.000000 0.34009222185
87.000000 0.38381351112
88.000000 0.38843856045
89.000000 0.36024796719
90.000000 0.34757175240
91.000000 0.36992846411
92.000000 0.30072995218
93.000000 0.31390831331
94.000000 0.29479949479
95.000000 0.25710710014
96.000000 0.30707786379
97.000000 0.40020929297
98.000000 0.36271632522
99.000000 0.31151857126
100.000000 0.25908916600
101.000000 0.29422189002
102.000000 0.31993044825
103.000000 0.31979247284
104.000000 0.26976064561
105.000000 0.23901539972
106.000000 0.27604345379
107.000000 0.28285039750
108.000000 0.29903706645
109.000000 0.30955598417
110.000000 0.27398876009
111.000000 0.26725086377
112.000000 0.25144285002
113.000000 0.23688681790
114.000000 0.18323073808
115.000000 0.21253865449
116.000000 0.27067397748
117.000000 0.22353773997
118.000000 0.26189740789
119.000000 0.22773001165
120.000000 0.18145434984
121.000000 0.17209002009
122.000000 0.17532691381
123.000000 0.15520526926
124.000000 0.16327586170
125.000000 0.16955358901
126.000000 0.12346486423
127.000000 0.11338866509
128.000000 0.24460206449
129.000000 0.12285737786
130.000000 0.13236185691
131.000000 0.24883541271
132.000000 0.10239403794
133.000000 0.20574039044
134.000000 0.10699374802
135.000000 0.23175420034
136.000000 0.11238387350
137.000000 0.24643022177
138.000000 0.10291350087
139.000000 0.24316587012
140.000000 0.08867681085
141.000000 0.15259099976
142.000000 0.19076591043
143.000000 0.09991300768
144.000000 0.21098928254
145.000000 0.11137201196
146.000000 0.09796996376
147.000000 0.23268973192
148.000000 0.08338256678
149.000000 0.11233918698
150.000000 0.23129970199
151.000000 0.09425506357
152.000000 0.08485819930
153.000000 0.17413429292
154.000000 0.15349654474
155.000000 0.06534803903
156.000000 0.13066343542
157.000000 0.18887056470
158.000000 0.07629191745
159.000000 0.07913999779
160.000000 0.19531069387
161.000000 0.13059284850
162.000000 0.06747366745
163.000000 0.06322284185
164.000000 0.16207565253
165.000000 0.16151588418
166.000000 0.06238000081
167.000000 0.06585376482
168.000000 0.13999991917
169.000000 0.12678177681
170.000000 0.05823491239
171.000000 0.06735077832
172.000000 0.12951412986
173.000000 0.14506467576
174.000000 0.06968202108
175.000000 0.04770054898
176.000000 0.08587766357
177.000000 0.15085616298
178.000000 0.08823327331
179.000000 0.04693011593
180.000000 0.05941328427
181.000000 0.11522253449
182.000000 0.12033052057
183.000000 0.06796490572
184.000000 0.04211350626
185.000000 0.05699035602
186.000000 0.11072202755
187.000000 0.11435711161
188.000000 0.05822468552
189.000000 0.04064876094
190.000000 0.05506508515
191.000000 0.09331707588
192.000000 0.10562975606
193.000000 0.06366279235
194.000000 0.04419324674
195.000000 0.04634738522
196.000000 0.07135356421
197.000000 0.09654980809
198.000000 0.07601794958
199.000000 0.05470809510
200.000000 0.03839137261
201.000000 0.04554427708
202.000000 0.08354246470
203.000000 0.08914466129
204.000000 0.06842814527
205.000000 0.03972420426
206.000000 0.03706125959
207.000000 0.05010260224
208.000000 0.07624743128
209.000000 0.08642780739
210.000000 0.05951398958
211.000000 0.03797785655
212.000000 0.03566008209
213.000000 0.04527329132
214.000000 0.07368042382
215.000000 0.08069510092
216.000000 0.05722493725
217.000000 0.03361699770
218.000000 0.03119946023
219.000000 0.05243669014
220.000000 0.06986678774
221.000000 0.07520223045
222.000000 0.05385998897
223.000000 0.03684861014
224.000000 0.02853817423
225.000000 0.04143544862
226.000000 0.05800790658
227.000000 0.06743726060
228.000000 0.05785519162
229.000000 0.04358658999
230.000000 0.02832534976
231.000000 0.03076125268
232.000000 0.04467609671
233.000000 0.06916462859
234.000000 0.05683451036
235.000000 0.03880690442
236.000000 0.02756548083
237.000000 0.02838244337
238.000000 0.04914523026
239.000000 0.05724874485
240.000000 0.04355026428
241.000000 0.02557328151
242.000000 0.02624888526
243.000000 0.05323227975
244.000000 0.04843478587
245.000000 0.04025924451
246.000000 0.02804056646
247.000000 0.02556726915
248.000000 0.04590393810
249.000000 0.05854202506
250.000000 0.03201867380
251.000000 0.02313336703
252.000000 0.03116387852
253.000000 0.06187714567
254.000000 0.03941921231
255.000000 0.05341255213
256.000000 0.02277671636
257.000000 0.02659834555
258.000000 0.04819565758
259.000000 0.04557318807
260.000000 0.07362551208
261.000000 0.02385324353
262.000000 0.03369134799
263.000000 0.02481783922
264.000000 0.08671774924
265.000000 0.03459528529
266.000000 0.05234475209
267.000000 0.02148844779
268.000000 0.03801669412
269.000000 0.03536435489
270.000000 0.04417021794
271.000000 0.05209973670
272.000000 0.03964753391
273.000000 0.03446165799
274.000000 0.02744637216
275.000000 0.04299411834
276.000000 0.02843357812
277.000000 0.07485847269
278.000000 0.04150436377
279.000000 0.04916764568
280.000000 0.03503149644
281.000000 0.02621755262
282.000000 0.05598315317
283.000000 0.04391718548
284.000000 0.07024326972
285.000000 0.06544506950
286.000000 0.04464454507
287.000000 0.05968637812
288.000000 0.03894898375
289.000000 0.03209041431
290.000000 0.08138138945
291.000000 0.09115804374
292.000000 0.04158663444
293.000000 0.06979061628
294.000000 0.03950061587
295.000000 0.03103743107
296.000000 0.09084175982
297.000000 0.05404139395
298.000000 0.03943116962
299.000000 0.05659659901
300.000000 0.02604446992
301.000000 0.02073132413
302.000000 0.03079018810
303.000000 0.02049308777
304.000000 0.02117536227
305.000000 0.02962647701
306.000000 0.01917797302
307.000000 0.00931566440
308.000000 0.01257221306
309.000000 0.00824138167
310.000000 0.00485928417
311.000000 0.00761393666
312.000000 0.01071549159
313.000000 0.00440679318
314.000000 0.00334648572
315.000000 0.00478092571
316.000000 0.00242604007
317.000000 0.00156954982
318.000000 0.00284961770
319.000000 0.00269266781
320.000000 0.00171708203
321.000000 0.00237698068
322.000000 0.00261901087
323.000000 0.00132369055
324.000000 0.00097830901
325.000000 0.00187375954
326.000000 0.00254588035
327.000000 0.00150778480
328.000000 0.00171962485
329.000000 0.00229355869
330.000000 0.00134525824
331.000000 0.00073299407
332.000000 0.00130554248
333.000000 0.00180994556
334.000000 0.00122437435
335.000000 0.00081527901
336.000000 0.00097310227
337.000000 0.00103297925
338.000000 0.00058223618
339.000000 0.00048226216
340.000000 0.00077045288
341.000000 0.00117904553
342.000000 0.00070549420
343.000000 0.00056563692
344.000000 0.00091011739
345.000000 0.00074776934
346.000000 0.00047576784
347.000000 0.00045841805
348.000000 0.00081152234
349.000000 0.00051387651
350.000000 0.00039129374
351.000000 0.00045621734
352.000000 0.00053275940
353.000000 0.00030331237
354.000000 0.00030754788
355.000000 0.00057679064
356.000000 0.00064676183
357.000000 0.00035841033
358.000000 0.00024570096
359.000000 0.00028832154
360.000000 0.00061386203
361.000000 0.00033670058
362.000000 0.00019756576
363.000000 0.00026207081
364.000000 0.00034391026
365.000000 0.00036248835
366.000000 0.00021625487
367.000000 0.00029742780
368.000000 0.00035774996
369.000000 0.00032593126
370.000000 0.00023433458
371.000000 0.00017745045
372.000000 0.00033947172
373.000000 0.00039310918
374.000000 0.00021649299
375.000000 0.00016256485
376.000000 0.00031466458
377.000000 0.00022738161
378.000000 0.00015407251
379.000000 0.00026928411
380.000000 0.00035205390
381.000000 0.00025538531
382.000000 0.00024367095
383.000000 0.00012884032
384.000000 0.00024504567
385.000000 0.00037509196
386.000000 0.00017551877
387.000000 0.00019758921
388.000000 0.00011473697
389.000000 0.00025436125
390.000000 0.00020546951
391.000000 0.00024438401
392.000000 0.00014486502
393.000000 0.00027861643
394.000000 0.00023319804
395.000000 0.00029057223
396.000000 0.00010404780
397.000000 0.00016748791
398.000000 0.00016066734
399.000000 0.00038837689
400.000000 0.00014007500
401.000000 0.00014314959
402.000000 0.00008478834
403.000000 0.00027910945
404.000000 0.00027134459
405.000000 0.00017788287
406.000000 0.00014506203
407.000000 0.00009477063
408.000000 0.00013972735
409.000000 0.00013073269
410.000000 0.00029836622
411.000000 0.00014771229
412.000000 0.00013436669
413.000000 0.00009664061
414.000000 0.00010717531
415.000000 0.00021697176
416.000000 0.00015125605
417.000000 0.00020956105
418.000000 0.00012497753
419.000000 0.00009645519
420.000000 0.00018603087
421.000000 0.00013690636
422.000000 0.00008897565
423.000000 0.00012161878
424.000000 0.00009295872
425.000000 0.00015723978
426.000000 0.00017096112
427.000000 0.00015691591
428.000000 0.00013518497
429.000000 0.00006091048
430.000000 0.00009845922
431.000000 0.00016051064
432.000000 0.00012458112
433.000000 0.00015900599
434.000000 0.00007538856
435.000000 0.00005534313
436.000000 0.00016340909
437.000000 0.00008128248
438.000000 0.00009395516
439.000000 0.00008259076
440.000000 0.00008872038
441.000000 0.00012752983
442.000000 0.00010061236
443.000000 0.00004748668
444.000000 0.00005600338
445.000000 0.00008622604
446.000000 0.00008344895
447.000000 0.00012226709
448.000000 0.00007536753
449.000000 0.00004540207
450.000000 0.00006513693
451.000000 0.00005306883
452.000000 0.00006205517
453.000000 0.00011359674
454.000000 0.00005315320
455.000000 0.00003551478
456.000000 0.00005518769
457.000000 0.00004102500
458.000000 0.00007114975
459.000000 0.00006933689
460.000000 0.00003758588
461.000000 0.00003590809
462.000000 0.00008123577
463.000000 0.00003758871
464.000000 0.00003105917
465.000000 0.00003931795
466.000000 0.00002902351
467.000000 0.00005124075
468.000000 0.00007350024
469.000000 0.00003240911
470.000000 0.00001994904
471.000000 0.00003363082
472.000000 0.00005873611
473.000000 0.00003596517
474.000000 0.00002943274
475.000000 0.00003197335
476.000000 0.00001828849
477.000000 0.00003205314
478.000000 0.00004531810
479.000000 0.00003055584
480.000000 0.00002554442
481.000000 0.00002931135
482.000000 0.00001877337
483.000000 0.00003043690
484.000000 0.00003878164
485.000000 0.00002611381
486.000000 0.00001473392
487.000000 0.00002333984
488.000000 0.00002636467
489.000000 0.00002144835
490.000000 0.00003089669
491.000000 0.00002384980
492.000000 0.00001327077
493.000000 0.00002190035
494.000000 0.00004460370
495.000000 0.00002597434
496.000000 0.00001821101
497.000000 0.00002482632
498.000000 0.00002175743
499.000000 0.00001076508
500.000000 0.00003779064
501.000000 0.00003803876
502.000000 0.00001440778
503.000000 0.00002496205
504.000000 0.00001310712
505.000000 0.00001359264
506.000000 0.00002520665
507.000000 0.00003059700
508.000000 0.00002123510
509.000000 0.00001045570
510.000000 0.00001731542
511.000000 0.00002777575
512.000000 0.00001703630
513.000000 0.00003028556
514.000000 0.00002688693
515.000000 0.00002131038
516.000000 0.00001068394
517.000000 0.00001496528
518.000000 0.00001934573
519.000000 0.00003990650
520.000000 0.00001795088
521.000000 0.00001232635
522.000000 0.00001626060
523.000000 0.00001774748
524.000000 0.00001842883
525.000000 0.00001477432
526.000000 0.00003300662
527.000000 0.00001740867
528.000000 0.00002035347
529.000000 0.00001008007
530.000000 0.00001837776
531.000000 0.00002384934
532.000000 0.00002568738
533.000000 0.00001457873
534.000000 0.00001292906
535.000000 0.00001618656
536.000000 0.00002190472
537.000000 0.00001388964
538.000000 0.00001394307
539.000000 0.00002508526
540.000000 0.00001593723
541.000000 0.00001656185
542.000000 0.00001059780
543.000000 0.00002578810
544.000000 0.00001947456
545.000000 0.00002005514
546.000000 0.00000995637
547.000000 0.00001313581
548.000000 0.00001853758
549.000000 0.00001464281
550.000000 0.00001912468
551.000000 0.00001639892
552.000000 0.00002598318
553.000000 0.00001248893
554.000000 0.00000893646
555.000000 0.00001669300
556.000000 0.00001786897
557.000000 0.00001656419
558.000000 0.00001838296
559.000000 0.00001516265
560.000000 0.00002250299
561.000000 0.00001095053
562.000000 0.00001181484
563.000000 0.00001582388
564.000000 0.00001737932
565.000000 0.00003152026
566.000000 0.00001504100
567.000000 0.00000974941
568.000000 0.00001339609
569.000000 0.00001552898
570.000000 0.00003933637
571.000000 0.00001399946
572.000000 0.00001013375
573.000000 0.00002341685
574.000000 0.00001697366
575.000000 0.00002232008
576.000000 0.00001383086
577.000000 0.00002512270
578.000000 0.00002617488
579.000000 0.00001402784
580.000000 0.00001503108
581.000000 0.00001445161
582.000000 0.00002296147
583.000000 0.00002751214
584.000000 0.00001174443
585.000000 0.00001201945
586.000000 0.00003415070
587.000000 0.00002011376
588.000000 0.00001640650
589.000000 0.00001779492
590.000000 0.00001426748
591.000000 0.00001563159
592.000000 0.00001785583
593.000000 0.00001427867
594.000000 0.00002383571
595.000000 0.00001512069
596.000000 0.00001904452
597.000000 0.00001543457
598.000000 0.00000906844
599.000000 0.00001921360
600.000000 0.00002985470
601.000000 0.00001916792
602.000000 0.00001695176
603.000000 0.00000759069
604.000000 0.00001271838
605.000000 0.00002053045
606.000000 0.00001613804
607.000000 0.00002055173
608.000000 0.00000993066
609.000000 0.00001183934
610.000000 0.00001689966
611.000000 0.00001300916
612.000000 0.00001554580
613.000000 0.00001186218
614.000000 0.00002335274
615.000000 0.00002231753
616.000000 0.00000870809
617.000000 0.00000887185
618.000000 0.00001735225
619.000000 0.00001661178
620.000000 0.00001836758
621.000000 0.00001642550
622.000000 0.00000784693
623.000000 0.00000800531
624.000000 0.00002558363
625.000000 0.00002408726
626.000000 0.00000805927
627.000000 0.00001179779
628.000000 0.00001419133
629.000000 0.00001309257
630.000000 0.00001909074
631.000000 0.00001511576
632.000000 0.00001178486
633.000000 0.00001524683
634.000000 0.00001441528
635.000000 0.00001168434
636.000000 0.00000814640
637.000000 0.00002528537
638.000000 0.00002300599
639.000000 0.00001748102
640.000000 0.00000812914
641.000000 0.00001613252
642.000000 0.00001337007
643.000000 0.00001822200
644.000000 0.00002092584
645.000000 0.00001817671
646.000000 0.00001126004
647.000000 0.00000834939
648.000000 0.00002724444
649.000000 0.00001538475
650.000000 0.00001675170
651.000000 0.00001585951
652.000000 0.00001161073
653.000000 0.00001274509
654.000000 0.00001451369
655.000000 0.00001984785
656.000000 0.00000898530
657.000000 0.00001675682
658.000000 0.00002029641
659.000000 0.00002000105
660.000000 0.00000912897
661.000000 0.00001514541
662.000000 0.00001093721
663.000000 0.00001207311
664.000000 0.00001835982
665.000000 0.00002086509
666.000000 0.00000838673
667.000000 0.00000825845
668.000000 0.00001680874
669.000000 0.00002208671
670.000000 0.00001029516
671.000000 0.00000741218
672.000000 0.00001250569
673.000000 0.00001276505
674.000000 0.00001446283
675.000000 0.00001265026
676.000000 0.00001937454
677.000000 0.00000771808
678.000000 0.00000697169
679.000000 0.00000996035
680.000000 0.00001406951
681.000000 0.00002105020
682.000000 0.00000726798
683.000000 0.00000783655
684.000000 0.00000868792
685.000000 0.00000867608
686.000000 0.00001055941
687.000000 0.00001165717
688.000000 0.00001634727
689.000000 0.00001009997
690.000000 0.00000745980
691.000000 0.00000646982
692.000000 0.00000649666
693.000000 0.00001385075
694.000000 0.00001236285
695.000000 0.00001159170
696.000000 0.00000734782
697.000000 0.00000748400
698.000000 0.00000863767
699.000000 0.00000477015
700.000000 0.00001378521
701.000000 0.00001013447
702.000000 0.00000947358
703.000000 0.00000458483
704.000000 0.00000496540
705.000000 0.00001101742
706.000000 0.00000900421
707.000000 0.00000676107
708.000000 0.00000516234
709.000000 0.00000819977
710.000000 0.00000476885
711.000000 0.00000896705
712.000000 0.00000748783
713.000000 0.00000976951
714.000000 0.00000641683
715.000000 0.00000617511
716.000000 0.00000870648
717.000000 0.00000405564
718.000000 0.00000685894
719.000000 0.00000794505
720.000000 0.00000723168
721.000000 0.00000738738
722.000000 0.00000942091
723.000000 0.00000957125
724.000000 0.00000479206
725.000000 0.00000389450
726.000000 0.00000868912
727.000000 0.00001578737
728.000000 0.00000597697
729.000000 0.00000464820
730.000000 0.00000439997
731.000000 0.00000619282
732.000000 0.00001243813
733.000000 0.00000516831
734.000000 0.00000674077
735.000000 0.00000475452
736.000000 0.00000516412
737.000000 0.00000653493
738.000000 0.00000558413
739.000000 0.00001083754
740.000000 0.00000666742
741.000000 0.00000579057
742.000000 0.00000622631
743.000000 0.00000446791
744.000000 0.00000848997
745.000000 0.00000624534
746.000000 0.00000363720
747.000000 0.00000917444
748.000000 0.00000916753
749.000000 0.00000359006
750.000000 0.00000630024
751.000000 0.00000414043
752.000000 0.00000389555
753.000000 0.00001010599
754.000000 0.00000762383
755.000000 0.00000353395
756.000000 0.00000456792
757.000000 0.00000458417
758.000000 0.00000419499
759.000000 0.00000838913
760.000000 0.00000402617
761.000000 0.00000742105
762.000000 0.00000592285
763.000000 0.00000360992
764.000000 0.00000370529
765.000000 0.00000415907
766.000000 0.00000412707
767.000000 0.00000659345
768.000000 0.00000819565
769.000000 0.00000288368
770.000000 0.00000425792
771.000000 0.00000325028
772.000000 0.00000334946
773.000000 0.00000630488
774.000000 0.00000426626
775.000000 0.00000389043
776.000000 0.00000317306
777.000000 0.00000488431
778.000000 0.00000298949
779.000000 0.00000402818
780.000000 0.00000283144
781.000000 0.00000350708
782.000000 0.00000564706
783.000000 0.00000256163
784.000000 0.00000323773
785.000000 0.00000403722
786.000000 0.00000508251
787.000000 0.00000266321
788.000000 0.00000318956
789.000000 0.00000198809
790.000000 0.00000334346
791.000000 0.00000408601
792.000000 0.00000593042
793.000000 0.00000187495
794.000000 0.00000210243
795.000000 0.00000278024
796.000000 0.00000341931
797.000000 0.00000347882
798.000000 0.00000529361
799.000000 0.00000156305
800.000000 0.00000194067
801.000000 0.00000306397
802.000000 0.00000507158
803.000000 0.00000235734
804.000000 0.00000162275
805.000000 0.00000193290
806.000000 0.00000277543
807.000000 0.00000476295
808.000000 0.00000244780
809.000000 0.00000216877
810.000000 0.00000186318
811.000000 0.00000227987
812.000000 0.00000188929
813.000000 0.00000343918
814.000000 0.00000207198
815.000000 0.00000202793
816.000000 0.00000305754
817.000000 0.00000297272
818.000000 0.00000158905
819.000000 0.00000132580
820.000000 0.00000357045
821.000000 0.00000277728
822.000000 0.00000124881
823.000000 0.00000235176
824.000000 0.00000281842
825.000000 0.00000184106
826.000000 0.00000190338
827.000000 0.00000184619
828.000000 0.00000158129
829.000000 0.00000259709
830.000000 0.00000290127
831.000000 0.00000170731
832.000000 0.00000194507
833.000000 0.00000194900
834.000000 0.00000181221
835.000000 0.00000111849
836.000000 0.00000274362
837.000000 0.00000206425
838.000000 0.00000256935
839.000000 0.00000199172
840.000000 0.00000162098
841.000000 0.00000096258
842.000000 0.00000183425
843.000000 0.00000403619
844.000000 0.00000166915
845.000000 0.00000130569
846.000000 0.00000104698
847.000000 0.00000147071
848.000000 0.00000175986
849.000000 0.00000212783
850.000000 0.00000180748
851.000000 0.00000163975
852.000000 0.00000145956
853.000000 0.00000101343
854.000000 0.00000146437
855.000000 0.00000137619
856.000000 0.00000166691
857.000000 0.00000118400
858.000000 0.00000176811
859.000000 0.00000105263
860.000000 0.00000084944
861.000000 0.00000162613
862.000000 0.00000240992
863.000000 0.00000293640
864.000000 0.00000095077
865.000000 0.00000090679
866.000000 0.00000149721
867.000000 0.00000159925
868.000000 0.00000207069
869.000000 0.00000224005
870.000000 0.00000133280
871.000000 0.00000132009
872.000000 0.00000088718
873.000000 0.00000084500
874.000000 0.00000256780
875.000000 0.00000114370
876.000000 0.00000108504
877.000000 0.00000078638
878.000000 0.00000096665
879.000000 0.00000157722
880.000000 0.00000116568
881.000000 0.00000157330
882.000000 0.00000144136
883.000000 0.00000067479
884.000000 0.00000061009
885.000000 0.00000124510
886.000000 0.00000146627
887.000000 0.00000128390
888.000000 0.00000085936
889.000000 0.00000069661
890.000000 0.00000135013
891.000000 0.00000083854
892.000000 0.00000064478
893.000000 0.00000118715
894.000000 0.00000082126
895.000000 0.00000098508
896.000000 0.00000103408
897.000000 0.00000100164
898.000000 0.00000078662
899.000000 0.00000047543
900.000000 0.00000087512
901.000000 0.00000147397
902.000000 0.00000097896
903.000000 0.00000036943
904.000000 0.00000087462
905.000000 0.00000124247
906.000000 0.00000078407
907.000000 0.00000101266
908.000000 0.00000043362
909.000000 0.00000082939
910.000000 0.00000108790
911.000000 0.00000095385
912.000000 0.00000049969
913.000000 0.00000089579
914.000000 0.00000084135
915.000000 0.00000084999
916.000000 0.00000070169
917.000000 0.00000122904
918.000000 0.00000066038
919.000000 0.00000046725
920.000000 0.00000069213
921.000000 0.00000127754
922.000000 0.00000059133
923.000000 0.00000061606
924.000000 0.00000074473
925.000000 0.00000081599
926.000000 0.00000092754
927.000000 0.00000042529
928.000000 0.00000066961
929.000000 0.00000089019
930.000000 0.00000081656
931.000000 0.00000066532
932.000000 0.00000101550
933.000000 0.00000077659
934.000000 0.00000047902
935.000000 0.00000060377
936.000000 0.00000075948
937.000000 0.00000104574
938.000000 0.00000103250
939.000000 0.00000102779
940.000000 0.00000042955
941.000000 0.00000041179
942.000000 0.00000130920
943.000000 0.00000106258
944.000000 0.00000071495
945.000000 0.00000048007
946.000000 0.00000050475
947.000000 0.00000048700
948.000000 0.00000075439
949.000000 0.00000106035
950.000000 0.00000074062
951.000000 0.00000062691
952.000000 0.00000057611
953.000000 0.00000055359
954.000000 0.00000052934
955.000000 0.00000070286
956.000000 0.00000065713
957.000000 0.00000078545
958.000000 0.00000079649
959.000000 0.00000091446
960.000000 0.00000039100
961.000000 0.00000039950
962.000000 0.00000058801
963.000000 0.00000086912
964.000000 0.00000059559
965.000000 0.00000077884
966.000000 0.00000039509
967.000000 0.00000049356
968.000000 0.00000035738
969.000000 0.00000051389
970.000000 0.00000096256
971.000000 0.00000030195
972.000000 0.00000029848
973.000000 0.00000110245
974.000000 0.00000051097
975.000000 0.00000047935
976.000000 0.00000039329
977.000000 0.00000035483
978.000000 0.00000039929
979.000000 0.00000057494
980.000000 0.00000043177
981.000000 0.00000041290
982.000000 0.00000042789
983.000000 0.00000040423
984.000000 0.00000024996
985.000000 0.00000044789
986.000000 0.00000062846
987.000000 0.00000030985
988.000000 0.00000045247
989.000000 0.00000026837
990.000000 0.00000028096
991.000000 0.00000036410
992.000000 0.00000070660
993.000000 0.00000024743
994.000000 0.00000019326
995.000000 0.00000040638
996.000000 0.00000037861
997.000000 0.00000029979
998.000000 0.00000028633
999.000000 0.00000034198
1000.000000 0.00000037072
1001.000000 0.00000017555
1002.000000 0.00000019018
1003.000000 0.00000036699
1004.000000 0.00000038223
1005.000000 0.00000027214
1006.000000 0.00000020609
1007.000000 0.00000019696
1008.000000 0.00000025158
1009.000000 0.00000032495
1010.000000 0.00000024480
1011.000000 0.00000015243
1012.000000 0.00000026001
1013.000000 0.00000034074
1014.000000 0.00000022370
1015.000000 0.00000029261
1016.000000 0.00000015397
1017.000000 0.00000016220
1018.000000 0.00000019265
1019.000000 0.00000025956
1020.000000 0.00000041750
1021.000000 0.00000013367
1022.000000 0.00000010539
1023.000000 0.00000022301
1024.000000 0.00000027022
1025.000000 0.00000023651
1026.000000 0.00000016250
1027.000000 0.00000011877
1028.000000 0.00000011969
1029.000000 0.00000020256
1030.000000 0.00000026949
1031.000000 0.00000016441
1032.000000 0.00000013214
1033.000000 0.00000010856
1034.000000 0.00000016501
1035.000000 0.00000021187
1036.000000 0.00000029047
1037.000000 0.00000014970
1038.000000 0.00000023519
1039.000000 0.00000009922
1040.000000 0.00000013414
1041.000000 0.00000020115
1042.000000 0.00000022258
1043.000000 0.00000011578
1044.000000 0.00000026146
1045.000000 0.00000021470
1046.000000 0.00000012093
1047.000000 0.00000009127
1048.000000 0.00000019270
1049.000000 0.00000019523
1050.000000 0.00000021590
1051.000000 0.00000014363
1052.000000 0.00000011897
1053.000000 0.00000015088
1054.000000 0.00000025164
1055.000000 0.00000010585
1056.000000 0.00000011653
1057.000000 0.00000014099
1058.000000 0.00000019754
1059.000000 0.00000024379
1060.000000 0.00000012880
1061.000000 0.00000011493
1062.000000 0.00000010094
1063.000000 0.00000015530
1064.000000 0.00000010814
1065.000000 0.00000028259
1066.000000 0.00000009431
1067.000000 0.00000007110
1068.000000 0.00000018825
1069.000000 0.00000014999
1070.000000 0.00000012861
1071.000000 0.00000017647
1072.000000 0.00000011487
1073.000000 0.00000012098
1074.000000 0.00000011379
1075.000000 0.00000009340
1076.000000 0.00000010369
1077.000000 0.00000014783
1078.000000 0.00000012869
1079.000000 0.00000012541
1080.000000 0.00000013286
1081.000000 0.00000014293
1082.000000 0.00000007747
1083.000000 0.00000005934
1084.000000 0.00000011238
1085.000000 0.00000012282
1086.000000 0.00000008529
1087.000000 0.00000007820
1088.000000 0.00000011466
1089.000000 0.00000005475
1090.000000 0.00000011384
1091.000000 0.00000010167
1092.000000 0.00000010900
1093.000000 0.00000009571
1094.000000 0.00000009623
1095.000000 0.00000007843
1096.000000 0.00000008117
1097.000000 0.00000006436
1098.000000 0.00000006679
1099.000000 0.00000011271
1100.000000 0.00000007706
1101.000000 0.00000006193
1102.000000 0.00000006367
1103.000000 0.00000010188
1104.000000 0.00000013381
1105.000000 0.00000005216
1106.000000 0.00000005912
1107.000000 0.00000015338
1108.000000 0.00000009537
1109.000000 0.00000005601
1110.000000 0.00000005764
1111.000000 0.00000004706
1112.000000 0.00000013019
1113.000000 0.00000004998
1114.000000 0.00000003792
1115.000000 0.00000007287
1116.000000 0.00000006797
1117.000000 0.00000009305
1118.000000 0.00000007602
1119.000000 0.00000006460
1120.000000 0.00000006183
1121.000000 0.00000003005
1122.000000 0.00000006562
1123.000000 0.00000009501
1124.000000 0.00000006826
1125.000000 0.00000005583
1126.000000 0.00000003443
1127.000000 0.00000004418
1128.000000 0.00000004233
1129.000000 0.00000007614
1130.000000 0.00000008620
1131.000000 0.00000003955
1132.000000 0.00000003899
1133.000000 0.00000002915
1134.000000 0.00000005391
1135.000000 0.00000006847
1136.000000 0.00000006263
1137.000000 0.00000002733
1138.000000 0.00000002996
1139.000000 0.00000004835
1140.000000 0.00000005827
1141.000000 0.00000004040
1142.000000 0.00000002695
1143.000000 0.00000003290
1144.000000 0.00000004038
1145.000000 0.00000004429
1146.000000 0.00000002962
1147.000000 0.00000003354
1148.000000 0.00000005340
1149.000000 0.00000002309
1150.000000 0.00000002805
1151.000000 0.00000003655
1152.000000 0.00000003474
1153.000000 0.00000002117
1154.000000 0.00000003311
1155.000000 0.00000002993
1156.000000 0.00000003419
1157.000000 0.00000002885
1158.000000 0.00000001697
1159.000000 0.00000002555
1160.000000 0.00000002506
1161.000000 0.00000004828
1162.000000 0.00000001720
1163.000000 0.00000002293
1164.000000 0.00000002245
1165.000000 0.00000002472
1166.000000 0.00000002346
1167.000000 0.00000002174
1168.000000 0.00000002071
1169.000000 0.00000002709
1170.000000 0.00000001662
1171.000000 0.00000002105
1172.000000 0.00000001936
1173.000000 0.00000003029
1174.000000 0.00000002942
1175.000000 0.00000001186
1176.000000 0.00000001595
1177.000000 0.00000001732
1178.000000 0.00000002615
1179.000000 0.00000003145
1180.000000 0.00000002824
1181.000000 0.00000001425
1182.000000 0.00000001845
1183.000000 0.00000001888
1184.000000 0.00000001636
1185.000000 0.00000001692
1186.000000 0.00000002504
1187.000000 0.00000002602
1188.000000 0.00000003364
1189.000000 0.00000000954
1190.000000 0.00000001280
1191.000000 0.00000002312
1192.000000 0.00000003450
1193.000000 0.00000002172
1194.000000 0.00000001687
1195.000000 0.00000000996
1196.000000 0.00000001847
1197.000000 0.00000002559
1198.000000 0.00000002175
1199.000000 0.00000001327
1200.000000 0.00000002450
1201.000000 0.00000001754
1202.000000 0.00000001856
1203.000000 0.00000002298
1204.000000 0.00000001565
1205.000000 0.00000001114
1206.000000 0.00000001470
1207.000000 0.00000003008
1208.000000 0.00000001337
1209.000000 0.00000001659
1210.000000 0.00000001336
1211.000000 0.00000001503
1212.000000 0.00000001648
1213.000000 0.00000001888
1214.000000 0.00000002931
1215.000000 0.00000001423
1216.000000 0.00000001849
1217.000000 0.00000000860
1218.000000 0.00000001434
1219.000000 0.00000002260
1220.000000 0.00000002576
1221.000000 0.00000001996
1222.000000 0.00000001443
1223.000000 0.00000000986
1224.000000 0.00000001227
1225.000000 0.00000001463
1226.000000 0.00000001913
1227.000000 0.00000001493
1228.000000 0.00000001203
1229.000000 0.00000001258
1230.000000 0.00000001131
1231.000000 0.00000001456
1232.000000 0.00000001202
1233.000000 0.00000001068
1234.000000 0.00000001183
1235.000000 0.00000000920
1236.000000 0.00000000661
1237.000000 0.00000001587
1238.000000 0.00000002503
1239.000000 0.00000000771
1240.000000 0.00000000681
1241.000000 0.00000000808
1242.000000 0.00000001733
1243.000000 0.00000001277
1244.000000 0.00000001395
1245.000000 0.00000000569
1246.000000 0.00000000744
1247.000000 0.00000000917
1248.000000 0.00000001548
1249.000000 0.00000000805
1250.000000 0.00000000686
1251.000000 0.00000000694
1252.000000 0.00000000559
1253.000000 0.00000000830
1254.000000 0.00000001339
1255.000000 0.00000000808
1256.000000 0.00000000436
1257.000000 0.00000000648
1258.000000 0.00000000539
1259.000000 0.00000001286
1260.000000 0.00000001001
1261.000000 0.00000000298
1262.000000 0.00000000809
1263.000000 0.00000000637
1264.000000 0.00000000621
1265.000000 0.00000000852
1266.000000 0.00000000571
1267.000000 0.00000000322
1268.000000 0.00000000802
1269.000000 0.00000000576
1270.000000 0.00000000344
1271.000000 0.00000000645
1272.000000 0.00000000718
1273.000000 0.00000000460
1274.000000 0.00000000354
1275.000000 0.00000000591
1276.000000 0.00000000453
1277.000000 0.00000000463
1278.000000 0.00000000637
1279.000000 0.00000000419
1280.000000 0.00000000387
1281.000000 0.00000000572
1282.000000 0.00000000301
1283.000000 0.00000000569
1284.000000 0.00000000439
1285.000000 0.00000000312
1286.000000 0.00000000234
1287.000000 0.00000000332
1288.000000 0.00000000873
1289.000000 0.00000000337
1290.000000 0.00000000241
1291.000000 0.00000000279
1292.000000 0.00000000253
1293.000000 0.00000000466
1294.000000 0.00000000480
1295.000000 0.00000000362
1296.000000 0.00000000222
1297.000000 0.00000000223
1298.000000 0.00000000352
1299.000000 0.00000000197
1300.000000 0.00000000327
1301.000000 0.00000000273
1302.000000 0.00000000338
1303.000000 0.00000000349
1304.000000 0.00000000211
1305.000000 0.00000000187
1306.000000 0.00000000246
1307.000000 0.00000000299
1308.000000 0.00000000229
1309.000000 0.00000000219
1310.000000 0.00000000181
1311.000000 0.00000000343
1312.000000 0.00000000260
1313.000000 0.00000000219
1314.000000 0.00000000194
1315.000000 0.00000000166
1316.000000 0.00000000142
1317.000000 0.00000000200
1318.000000 0.00000000271
1319.000000 0.00000000302
1320.000000 0.00000000108
1321.000000 0.00000000116
1322.000000 0.00000000219
1323.000000 0.00000000350
1324.000000 0.00000000175
1325.000000 0.00000000158
1326.000000 0.00000000126
1327.000000 0.00000000184
1328.000000 0.00000000196
1329.000000 0.00000000145
1330.000000 0.00000000126
1331.000000 0.00000000180
1332.000000 0.00000000209
1333.000000 0.00000000200
1334.000000 0.00000000082
1335.000000 0.00000000112
1336.000000 0.00000000126
1337.000000 0.00000000158
1338.000000 0.00000000152
1339.000000 0.00000000222
1340.000000 0.00000000104
1341.000000 0.00000000081
1342.000000 0.00000000096
1343.000000 0.00000000093
1344.000000 0.00000000094
1345.000000 0.00000000146
1346.000000 0.00000000142
1347.000000 0.00000000151
1348.000000 0.00000000055
1349.000000 0.00000000053
1350.000000 0.00000000175
1351.000000 0.00000000114
1352.000000 0.00000000110
1353.000000 0.00000000044
1354.000000 0.00000000093
1355.000000 0.00000000063
1356.000000 0.00000000197
1357.000000 0.00000000063
1358.000000 0.00000000043
1359.000000 0.00000000102
1360.000000 0.00000000102
1361.000000 0.00000000055
1362.000000 0.00000000079
1363.000000 0.00000000068
1364.000000 0.00000000072
1365.000000 0.00000000058
1366.000000 0.00000000076
1367.000000 0.00000000057
1368.000000 0.00000000047
1369.000000 0.00000000040
1370.000000 0.00000000078
1371.000000 0.00000000087
1372.000000 0.00000000072
1373.000000 0.00000000026
1374.000000 0.00000000061
1375.000000 0.00000000049
1376.000000 0.00000000057
1377.000000 0.00000000070
1378.000000 0.00000000031
1379.000000 0.00000000036
1380.000000 0.00000000051
1381.000000 0.00000000035
1382.000000 0.00000000064
1383.000000 0.00000000048
1384.000000 0.00000000051
1385.000000 0.00000000037
1386.000000 0.00000000025
1387.000000 0.00000000026
1388.000000 0.00000000043
1389.000000 0.00000000067
1390.000000 0.00000000038
1391.000000 0.00000000018
1392.000000 0.00000000028
1393.000000 0.00000000025
1394.000000 0.00000000027
1395.000000 0.00000000047
1396.000000 0.00000000018
1397.000000 0.00000000027
1398.000000 0.00000000023
1399.000000 0.00000000028
1400.000000 0.00000000020
1401.000000 0.00000000024
1402.000000 0.00000000034
1403.000000 0.00000000014
1404.000000 0.00000000034
1405.000000 0.00000000024
1406.000000 0.00000000019
1407.000000 0.00000000028
1408.000000 0.00000000016
1409.000000 0.00000000016
1410.000000 0.00000000033
1411.000000 0.00000000025
1412.000000 0.00000000028
1413.000000 0.00000000021
1414.000000 0.00000000010
1415.000000 0.00000000021
1416.000000 0.00000000035
1417.000000 0.00000000018
1418.000000 0.00000000010
1419.000000 0.00000000018
1420.000000 0.00000000015
1421.000000 0.00000000033
1422.000000 0.00000000020
1423.000000 0.00000000015
1424.000000 0.00000000014
1425.000000 0.00000000019
1426.000000 0.00000000021
1427.000000 0.00000000011
1428.000000 0.00000000013
1429.000000 0.00000000035
1430.000000 0.00000000010
1431.000000 0.00000000012
1432.000000 0.00000000018
1433.000000 0.00000000011
1434.000000 0.00000000011
1435.000000 0.00000000013
1436.000000 0.00000000025
1437.000000 0.00000000012
1438.000000 0.00000000011
1439.000000 0.00000000014
1440.000000 0.00000000012
1441.000000 0.00000000010


==> data/CG_ic0_D100.tex <==
0.000000 1.00000000000
1.000000 0.29598873951
2.000000 0.22351974396
3.000000 0.19352493279
4.000000 0.16299428271
5.000000 0.13467682288
6.000000 0.11502069609
7.000000 0.08991725877
8.000000 0.06975918940
9.000000 0.05543310616
10.000000 0.04250613818
11.000000 0.03309832742
12.000000 0.02650516452
13.000000 0.02159256861
14.000000 0.01850004502
15.000000 0.01712709067
16.000000 0.01550505152
17.000000 0.01576994186
18.000000 0.01622567635
19.000000 0.01659942191
20.000000 0.01256786247
21.000000 0.00596714575
22.000000 0.00212086259
23.000000 0.00075200783
24.000000 0.00058605958
25.000000 0.00058803019
26.000000 0.00038414994
27.000000 0.00041392622
28.000000 0.00026541996
29.000000 0.00021974302
30.000000 0.00019422746
31.000000 0.00015878444
32.000000 0.00016010840
33.000000 0.00014343864
34.000000 0.00014830797
35.000000 0.00014085470
36.000000 0.00014938972
37.000000 0.00013018922
38.000000 0.00012589064
39.000000 0.00010461816
40.000000 0.00009616319
41.000000 0.00007769674
42.000000 0.00007820522
43.000000 0.00007143619
44.000000 0.00007147010
45.000000 0.00006001380
46.000000 0.00005849950
47.000000 0.00005248641
48.000000 0.00004298655
49.000000 0.00003631760
50.000000 0.00003029733
51.000000 0.00002589230
52.000000 0.00002350655
53.000000 0.00002076668
54.000000 0.00001836723
55.000000 0.00001718925
56.000000 0.00001553679
57.000000 0.00001309434
58.000000 0.00001079500
59.000000 0.00000852150
60.000000 0.00000669867
61.000000 0.00000470631
62.000000 0.00000419600
63.000000 0.00000338083
64.000000 0.00000265052
65.000000 0.00000206542
66.000000 0.00000166879
67.000000 0.00000148080
68.000000 0.00000121381
69.000000 0.00000096520
70.000000 0.00000080651
71.000000 0.00000062783
72.000000 0.00000052058
73.000000 0.00000040884
74.000000 0.00000032452
75.000000 0.00000027618
76.000000 0.00000020439
77.000000 0.00000014840
78.000000 0.00000010218
79.000000 0.00000008029
80.000000 0.00000006778
81.000000 0.00000006095
82.000000 0.00000004787
83.000000 0.00000003789
84.000000 0.00000002971
85.000000 0.00000002027
86.000000 0.00000001391
87.000000 0.00000000937
88.000000 0.00000000619
89.000000 0.00000000398
90.000000 0.00000000250
91.000000 0.00000000172
92.000000 0.00000000118
93.000000 0.00000000078
94.000000 0.00000000062
95.000000 0.00000000053
96.000000 0.00000000042
97.000000 0.00000000030
98.000000 0.00000000021
99.000000 0.00000000015
100.000000 0.00000000010
101.000000 0.00000000007


==> data/CG_ic0_D1000.tex <==
0.000000 1.00000000000
1.000000 0.30101181830
2.000000 0.22171084962
3.000000 0.20064024072
4.000000 0.16216791497
5.000000 0.15450704577
6.000000 0.12240173165
7.000000 0.10548664992
8.000000 0.08307082638
9.000000 0.06311263625
10.000000 0.05551804423
11.000000 0.04506839529
12.000000 0.03687620669
13.000000 0.02909479261
14.000000 0.02510095602
15.000000 0.02213123847
16.000000 0.01967168299
17.000000 0.01829954787
18.000000 0.01810862621
19.000000 0.01757854801
20.000000 0.01793310894
21.000000 0.01822031283
22.000000 0.01589628810
23.000000 0.00962896799
24.000000 0.00443151041
25.000000 0.00179219600
26.000000 0.00070602433
27.000000 0.00046365635
28.000000 0.00043205868
29.000000 0.00030184950
30.000000 0.00024303035
31.000000 0.00025667168
32.000000 0.00018934749
33.000000 0.00016489675
34.000000 0.00013455248
35.000000 0.00010262942
36.000000 0.00009929172
37.000000 0.00008096462
38.000000 0.00006617768
39.000000 0.00005965342
40.000000 0.00004936838
41.000000 0.00004558183
42.000000 0.00003975005
43.000000 0.00003408125
44.000000 0.00002639901
45.000000 0.00002105631
46.000000 0.00001848423
47.000000 0.00001475301
48.000000 0.00001342301
49.000000 0.00001116705
50.000000 0.00001089065
51.000000 0.00000943803
52.000000 0.00000935149
53.000000 0.00000842925
54.000000 0.00000699889
55.000000 0.00000576874
56.000000 0.00000496902
57.000000 0.00000405535
58.000000 0.00000314005
59.000000 0.00000279407
60.000000 0.00000220253
61.000000 0.00000179552
62.000000 0.00000150709
63.000000 0.00000126875
64.000000 0.00000108917
65.000000 0.00000104630
66.000000 0.00000098233
67.000000 0.00000095511
68.000000 0.00000081777
69.000000 0.00000082658
70.000000 0.00000083553
71.000000 0.00000080622
72.000000 0.00000072993
73.000000 0.00000064825
74.000000 0.00000061281
75.000000 0.00000068764
76.000000 0.00000062578
77.000000 0.00000057471
78.000000 0.00000052279
79.000000 0.00000048111
80.000000 0.00000039236
81.000000 0.00000031655
82.000000 0.00000027398
83.000000 0.00000021308
84.000000 0.00000016351
85.000000 0.00000012296
86.000000 0.00000009389
87.000000 0.00000007241
88.000000 0.00000005091
89.000000 0.00000003824
90.000000 0.00000003416
91.000000 0.00000002807
92.000000 0.00000002304
93.000000 0.00000001917
94.000000 0.00000001427
95.000000 0.00000000959
96.000000 0.00000000739
97.000000 0.00000000585
98.000000 0.00000000444
99.000000 0.00000000354
100.000000 0.00000000242
101.000000 0.00000000169
102.000000 0.00000000125
103.000000 0.00000000087
104.000000 0.00000000066
105.000000 0.00000000049
106.000000 0.00000000041
107.000000 0.00000000034
108.000000 0.00000000027
109.000000 0.00000000019
110.000000 0.00000000013
111.000000 0.00000000010
112.000000 0.00000000007


==> data/CG_ic0_D10000.tex <==
0.000000 1.00000000000
1.000000 0.30581302798
2.000000 0.22151084541
3.000000 0.19512325823
4.000000 0.16844752492
5.000000 0.15245792461
6.000000 0.12946571226
7.000000 0.10824107730
8.000000 0.08650248158
9.000000 0.07332763267
10.000000 0.06372796238
11.000000 0.05432443032
12.000000 0.04730670468
13.000000 0.04246583048
14.000000 0.03386693063
15.000000 0.02771759185
16.000000 0.02472948405
17.000000 0.02290567402
18.000000 0.02123637598
19.000000 0.02060614540
20.000000 0.02092338142
21.000000 0.02009003832
22.000000 0.02114108588
23.000000 0.02082144466
24.000000 0.01359394474
25.000000 0.00724685894
26.000000 0.00322638243
27.000000 0.00112436644
28.000000 0.00055525693
29.000000 0.00055926776
30.000000 0.00047982331
31.000000 0.00034309155
32.000000 0.00034402691
33.000000 0.00026620919
34.000000 0.00018204401
35.000000 0.00017188470
36.000000 0.00012658132
37.000000 0.00010161181
38.000000 0.00008970791
39.000000 0.00006741155
40.000000 0.00005947256
41.000000 0.00004824029
42.000000 0.00004220240
43.000000 0.00003976988
44.000000 0.00003670567
45.000000 0.00003397992
46.000000 0.00003008918
47.000000 0.00002969078
48.000000 0.00002712777
49.000000 0.00002500974
50.000000 0.00002279591
51.000000 0.00001949459
52.000000 0.00001722230
53.000000 0.00001547530
54.000000 0.00001637035
55.000000 0.00001615232
56.000000 0.00001522800
57.000000 0.00001558165
58.000000 0.00001561241
59.000000 0.00001392669
60.000000 0.00001202532
61.000000 0.00000928967
62.000000 0.00000860500
63.000000 0.00000810498
64.000000 0.00000689761
65.000000 0.00000608302
66.000000 0.00000565699
67.000000 0.00000585882
68.000000 0.00000547902
69.000000 0.00000508094
70.000000 0.00000475489
71.000000 0.00000422430
72.000000 0.00000334072
73.000000 0.00000244174
74.000000 0.00000166112
75.000000 0.00000122309
76.000000 0.00000099851
77.000000 0.00000077009
78.000000 0.00000062643
79.000000 0.00000052176
80.000000 0.00000045311
81.000000 0.00000039316
82.000000 0.00000032528
83.000000 0.00000026963
84.000000 0.00000021895
85.000000 0.00000019203
86.000000 0.00000016528
87.000000 0.00000014250
88.000000 0.00000010986
89.000000 0.00000009416
90.000000 0.00000006964
91.000000 0.00000005190
92.000000 0.00000004209
93.000000 0.00000003534
94.000000 0.00000002975
95.000000 0.00000002468
96.000000 0.00000001931
97.000000 0.00000001517
98.000000 0.00000001161
99.000000 0.00000000886
100.000000 0.00000000682
101.000000 0.00000000499
102.000000 0.00000000381
103.000000 0.00000000297
104.000000 0.00000000235
105.000000 0.00000000184
106.000000 0.00000000153
107.000000 0.00000000121
108.000000 0.00000000091
109.000000 0.00000000073
110.000000 0.00000000057
111.000000 0.00000000043
112.000000 0.00000000034
113.000000 0.00000000026
114.000000 0.00000000020
115.000000 0.00000000017
116.000000 0.00000000015
117.000000 0.00000000014
118.000000 0.00000000012
119.000000 0.00000000011
120.000000 0.00000000008


==> data/CG_ic0_D100000.tex <==
0.000000 1.00000000000
1.000000 0.30177185997
2.000000 0.21829889907
3.000000 0.19149305452
4.000000 0.16792748505
5.000000 0.15176626723
6.000000 0.12782317295
7.000000 0.10552961294
8.000000 0.08638592334
9.000000 0.07809501006
10.000000 0.06084384357
11.000000 0.05367812299
12.000000 0.04913283161
13.000000 0.04149390660
14.000000 0.03205334691
15.000000 0.02858091001
16.000000 0.02499196953
17.000000 0.02217648317
18.000000 0.02158076456
19.000000 0.02031259526
20.000000 0.01995135434
21.000000 0.02105143888
22.000000 0.02053973932
23.000000 0.02033820444
24.000000 0.01605746791
25.000000 0.00907823714
26.000000 0.00375246273
27.000000 0.00146038949
28.000000 0.00057633786
29.000000 0.00044572098
30.000000 0.00044356312
31.000000 0.00032806897
32.000000 0.00026775830
33.000000 0.00025169950
34.000000 0.00017094369
35.000000 0.00015033398
36.000000 0.00013394249
37.000000 0.00011324710
38.000000 0.00012676462
39.000000 0.00011436318
40.000000 0.00010585332
41.000000 0.00010803398
42.000000 0.00008774773
43.000000 0.00008719150
44.000000 0.00008615739
45.000000 0.00008543769
46.000000 0.00008069360
47.000000 0.00007759659
48.000000 0.00008007789
49.000000 0.00007206622
50.000000 0.00006856206
51.000000 0.00005513052
52.000000 0.00005435204
53.000000 0.00005050695
54.000000 0.00005103190
55.000000 0.00004339806
56.000000 0.00003431340
57.000000 0.00002703560
58.000000 0.00002309626
59.000000 0.00001979221
60.000000 0.00001719347
61.000000 0.00001474934
62.000000 0.00001257917
63.000000 0.00001105725
64.000000 0.00000943121
65.000000 0.00000797390
66.000000 0.00000723859
67.000000 0.00000671069
68.000000 0.00000661676
69.000000 0.00000580918
70.000000 0.00000530652
71.000000 0.00000497632
72.000000 0.00000395850
73.000000 0.00000308224
74.000000 0.00000220156
75.000000 0.00000151186
76.000000 0.00000109528
77.000000 0.00000090287
78.000000 0.00000077446
79.000000 0.00000063871
80.000000 0.00000052440
81.000000 0.00000042614
82.000000 0.00000034028
83.000000 0.00000028178
84.000000 0.00000025881
85.000000 0.00000023594
86.000000 0.00000021128
87.000000 0.00000017405
88.000000 0.00000013058
89.000000 0.00000009687
90.000000 0.00000008046
91.000000 0.00000006286
92.000000 0.00000004731
93.000000 0.00000003298
94.000000 0.00000002426
95.000000 0.00000001880
96.000000 0.00000001648
97.000000 0.00000001369
98.000000 0.00000001080
99.000000 0.00000000786
100.000000 0.00000000614
101.000000 0.00000000438
102.000000 0.00000000329
103.000000 0.00000000281
104.000000 0.00000000229
105.000000 0.00000000179
106.000000 0.00000000135
107.000000 0.00000000102
108.000000 0.00000000078
109.000000 0.00000000067
110.000000 0.00000000057
111.000000 0.00000000046
112.000000 0.00000000036
113.000000 0.00000000029
114.000000 0.00000000024
115.000000 0.00000000018
116.000000 0.00000000015
117.000000 0.00000000013
118.000000 0.00000000013
119.000000 0.00000000011
120.000000 0.00000000008


==> data/CG_ic0_D1000000.tex <==
0.000000 1.00000000000
1.000000 0.30184224932
2.000000 0.21805987202
3.000000 0.19179424959
4.000000 0.16817515279
5.000000 0.15205065467
6.000000 0.12798556624
7.000000 0.10565059156
8.000000 0.08642421583
9.000000 0.07822135969
10.000000 0.06081894490
11.000000 0.05361756767
12.000000 0.04922035142
13.000000 0.04134930769
14.000000 0.03201977497
15.000000 0.02864554147
16.000000 0.02495630601
17.000000 0.02225107794
18.000000 0.02162194072
19.000000 0.02033558259
20.000000 0.02001333682
21.000000 0.02108314574
22.000000 0.02053612362
23.000000 0.02039416458
24.000000 0.01605197742
25.000000 0.00908351388
26.000000 0.00377068780
27.000000 0.00145909922
28.000000 0.00057812387
29.000000 0.00044564744
30.000000 0.00044378192
31.000000 0.00032905069
32.000000 0.00026675595
33.000000 0.00025130431
34.000000 0.00017184690
35.000000 0.00014992151
36.000000 0.00013383296
37.000000 0.00011359943
38.000000 0.00012625613
39.000000 0.00011447365
40.000000 0.00010575360
41.000000 0.00010778002
42.000000 0.00008781652
43.000000 0.00008725730
44.000000 0.00008561316
45.000000 0.00008527777
46.000000 0.00008080905
47.000000 0.00007745212
48.000000 0.00007978550
49.000000 0.00007200277
50.000000 0.00006886471
51.000000 0.00005491183
52.000000 0.00005449150
53.000000 0.00005060652
54.000000 0.00005108620
55.000000 0.00004329037
56.000000 0.00003450610
57.000000 0.00002704614
58.000000 0.00002306085
59.000000 0.00001976287
60.000000 0.00001716904
61.000000 0.00001480499
62.000000 0.00001256155
63.000000 0.00001063414
64.000000 0.00000886366
65.000000 0.00000796382
66.000000 0.00000726721
67.000000 0.00000674597
68.000000 0.00000660463
69.000000 0.00000585924
70.000000 0.00000539540
71.000000 0.00000503250
72.000000 0.00000396274
73.000000 0.00000309765
74.000000 0.00000222469
75.000000 0.00000150898
76.000000 0.00000106716
77.000000 0.00000089392
78.000000 0.00000076868
79.000000 0.00000063956
80.000000 0.00000052994
81.000000 0.00000042743
82.000000 0.00000034045
83.000000 0.00000027994
84.000000 0.00000025591
85.000000 0.00000023687
86.000000 0.00000021296
87.000000 0.00000017594
88.000000 0.00000013277
89.000000 0.00000009766
90.000000 0.00000007905
91.000000 0.00000006223
92.000000 0.00000004701
93.000000 0.00000003296
94.000000 0.00000002502
95.000000 0.00000001947
96.000000 0.00000001725
97.000000 0.00000001378
98.000000 0.00000001099
99.000000 0.00000000794
100.000000 0.00000000612
101.000000 0.00000000438
102.000000 0.00000000321
103.000000 0.00000000266
104.000000 0.00000000230
105.000000 0.00000000187
106.000000 0.00000000138
107.000000 0.00000000103
108.000000 0.00000000076
109.000000 0.00000000060
110.000000 0.00000000052
111.000000 0.00000000041
112.000000 0.00000000032
113.000000 0.00000000027
114.000000 0.00000000021
115.000000 0.00000000017
116.000000 0.00000000015
117.000000 0.00000000013
118.000000 0.00000000012
119.000000 0.00000000011
120.000000 0.00000000008

